Rotation Invariant Quantization for Model Compression

Post-training Neural Network (NN) model compression is an attractive approach for deploying large, memory-consuming models on devices with limited memory resources. In this study, we investigate the rate-distortion tradeoff for NN model compression. First, we suggest a Rotation-Invariant Quantization (RIQ) technique that utilizes a single parameter to quantize the entire NN model, yielding a different rate at each layer, i.e., mixed-precision quantization. Then, we prove that our rotation-invariant approach is optimal in terms of compression. We rigorously evaluate RIQ and demonstrate its capabilities on various models and tasks. For example, RIQ facilitates $\times 19.4$ and $\times 52.9$ compression ratios on pre-trained VGG dense and pruned models, respectively, with $<0.4\%$ accuracy degradation. Code is available in \href{https://github.com/ehaleva/RIQ}{github.com/ehaleva/RIQ}.

==> sections/04_method.tex <==
\section{Rotation-invariant  Mixed-bit Quantization}\label{sec. frac}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we study an extended rate-distortion problem for NN models and characterize its minimizing distribution. In particular, first, we introduce a surrogate model that describes the quantization as rotation and scaling of the weights. This model indicates that the distribution of the quantized weights  in each layer is a rotation-invariant distribution \BB{Need to define what is rotation invariant distribution in terms of the model}.  Then, considering the cosine distance in \cref{eq: cosine dist def}, the surrogate model reveals that the rate-distortion is  minimized by a single-letter \BB{Rephrase to omit single letter} (scalar) product distribution, constructed as the product of the layers' rotation-invariant distribution. In words, the NN model's entropy is minimized when the quantization rates are independent of \emph{the orientation} of the weights $\rvw_{\ell}$ in each layer $\ell$. Finally, we design RIQ accordingly and suggest an efficient searching method to find this single-letter solution. 
%\YR{I think this paragraph is already exist as part of problem definition. No need to duplicate since we in limited space.}
%Given a pre-trained model $\gM$ with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, $\ghM$, for which the distance between the outputs is small.  To assess this distance, a sample $\rvx$ is sent through the original model and the quantized model, and the  \emph{cosine distance} between the outputs is measured according to \cref{eq: cosine dist def}. 
%In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable. Yet, since the cosine distance is a bounded measure, as we prove in the sequel, it still allows us to characterize the rate-distortion function, and in particular, the properties of the minimizing distribution.     % Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 

\subsection{Rate-Distortion Analysis of NN Models}
%%%%%%%%%%%%%%%%%%%
%\BB{The considered mixed-bit solution, where each layer is quantized at a different rate and the output distortion is smaller than a pre-defined threshold, resembles  the variable length, maximum distortion flavor of the rate-distortion problem \cite[Ch. 25.2]{polyanskiy2014lecture}.} %Accordingly, we state the following theorem. 

Extending \cref{eq: reconstruct w} to NN model quantization, where layer $\ell$ is encoded uniformly, yields
\begin{equation}
    \wwh_\ell= \left\lceil {\ww_\ell}/{\Delta_\ell}\right\rfloor \cdot \Delta_\ell
    % \rvwh_\ell= \left\lceil \frac{\rvw_\ell}{\Delta_\ell}\right\rfloor \cdot \Delta_\ell, \qquad \forall \ell=1,...,L.
    \label{eq: uniform vector quant}
\end{equation}
To analyze the rate-distortion of \cref{eq: uniform vector quant} for the cosine distance in \cref{eq: cosine dist def}, it is essential  to consider the resulting \emph{rotation and scale} in each layer. Accordingly, we define the following surrogate model.
\begin{model}\label{model}
Let $\ww_\ell$ be the realization of $\rvw_\ell$, and $\wwh_\ell$ denote its quantized representation. Let $\theta_\ell$ be the rotation angle from $\ww_\ell$ to  $\wwh_\ell$, such that $\inp{\frac{\ww_\ell}{\Vert \ww_\ell \Vert }}{\frac{\wwh_\ell}{\Vert \wwh_\ell \Vert}} = \cos(\theta_\ell)$. Then, 
% In particular, let $\theta_\ell$ be the rotation angle from $\ww_\ell$ to  $\wwh_\ell$, such that $\inp{\frac{\ww_\ell}{\Vert \ww_\ell \Vert }}{\frac{\wwh_\ell}{\Vert \wwh_\ell \Vert}} = \cos(\theta_\ell)$. Then, the relation between $\wwh_\ell$ and $\ww_\ell$  is given by the following surrogate model. 
\begin{equation}
\wwh_\ell=  \Vert \wwh_\ell  \Vert \cdot \rmU(\theta_\ell) \frac{\ww_\ell}{\Vert \ww_\ell \Vert}
    \label{eq: quantization to rotation}
\end{equation}
where $\rmU(\theta_\ell)$ is  an orthogonal transformation corresponding to the rotation by $\theta_\ell$ in the plane generated by $\ww_\ell$ and  $\wwh_\ell$.
\end{model}
Namely, to obtain $\wwh_\ell$, the transformation $\rmU(\theta_\ell)$ rotates the unit vector $\ww_\ell/\Vert \ww_\ell \Vert$ to align it with the direction of $\wwh_\ell$, and then, it is stretched into the length $\Vert\wwh_\ell\Vert$. Clearly, every result of \cref{eq: uniform vector quant} can be described in terms of rotation and scale, using \cref{eq: quantization to rotation}.   The merit of this model is merely its simple analysis. In practice, quantizing with \cref{eq: quantization to rotation} requires prior knowledge of the length $\Vert \wwh_\ell \Vert $, the rotation angle $\theta_\ell$, and the basis of the plane generated $ \wwh_\ell$ and $ \ww_\ell$, which are typically not available to the quantizer \BB{I would omit this statement}. Further, it is much simpler to implement quantization according to \cref{eq: uniform vector quant}. 

\BB{reviewer2: Why we need this statement about randomness? We just keep in mind that w follows some distribution.} Considering a random $\rvw_\ell$, the resulting $\rvwh_\ell$ and $\rtheta_\ell$ (and hence $\rmU(\rtheta_\ell)$) are random. Further, even when $\rvw_\ell$, $\Vert \rvwh_\ell \Vert$, and  $\rtheta_\ell$ are given, the transformation $\rmU(\rtheta_\ell)$ is random since the subspace in which it rotates about is random, and hence, the resulting $\rvwh_\ell$ is still random. Nevertheless,  the subspace in which $\rmU(\theta_\ell)$  rotates about does not affect the resulting cosine distance for a given $\rtheta_\ell$. In this case, $\rvwh_\ell$ agrees with any vector that resides on a cone that is $\theta_\ell$  away from $\rvw_\ell$, for which a single realization $\wwh_\ell$ matches \cref{eq: uniform vector quant} \BB{why 7 and not 8?}.  Namely, that is the point of intersection between this cone \BB{Not clear what cone you refer to. Need thorogh explanation.} and the subspace generated by $\ww_\ell$ and $\wwh_\ell$. Thus, any realization of $\wwh_\ell$ in \cref{eq: uniform vector quant} can be represented by \cref{eq: quantization to rotation}, yet, the opposite direction is not true in general \BB{I feel this is trivial and not need to be mentioned or talk about it earlier}. The indifference of the cosine distance to such rotations drives us to further examine the NN models' rate-distortion characteristics.  In the sequel, we analyze the surrogate model in \cref{eq: quantization to rotation} and find its rate-distortion minimizing distribution. Then, we reflect our findings into \cref{eq: uniform vector quant} to find suitable $\Delta_\ell$. \BB{I think whole this paragraph isn't clear. From where comes the indifference to rotations?}

%Since \cref{eq: uniform vector quant} is a subset of \cref{eq: quantization to rotation}, this yields a nearly optimal solution. 

% $\rtheta_\ell$ is a function of both $\ww_\ell$ and $\wwh_\ell$, and thus, for random $\rvw_\ell$ and $\rvwh_\ell$, the resulting $\rtheta_\ell$ is a random variable. 

% \cite{convay1982fast} showed that this structured quantization motivates a multidimensional lattice model,  where the reconstruction points (vectors) $\hat{\pmb{w}}_\ell$ reside on a lattice grid $\Ls(\rvb_1,\cdots,\rvb_{n_\ell}) \triangleq \brcs{\sum_{i=1}^{n_\ell} \zeta_i \rvb_i \vert \zeta_i \in \Z}$, generated by some  basis $\brcs{\rvb_i}_{i=1}^{n_\ell}$, where each $\rvb_i \in \R^{n_\ell}$. 
% Choosing the simplest basis of the form $\Delta_\ell \cdot \mathrm{I}_{n_\ell}$, where $\mathrm{I}_{n_\ell}$ is the $n_\ell \times n_\ell$ identity matrix, allows to associate every vector $\hat{\pmb{w}}_\ell$ with a set of integer coefficients $\zeta_i = \round{\frac{w_{\ell,i}}{\Delta_\ell}}$, for $1\leq i \leq  n_\ell$. 



% Moreover, the span of these basis vectors,     $\mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell}) \triangleq \brcs{\sum_{i=1}^{n_\ell} \zeta_i \rvb_i \vert \zeta_i \in \R}$, is continuous and thus  $\Ls(\rvb_1,\cdots,\rvb_{n_\ell}) \subset \mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell})$. Since this span covers all points in the lattice, we build a surrogate model that depicts the span and analyze it to provide insights on \cref{eq: uniform vector quant}. %and it is easier to analyze. Accordingly, we build a surrogate model  

% \begin{model}
% Let $\rvw_\ell$ be the weights of layer $\ell$, and $\rvwh_\ell$ denote the quantized representation of those weights. Let $\rtheta_\ell$ be the rotation angle from $\rvw_\ell$ to  $\rvwh_\ell$, such that $\inp{\frac{\rvw_\ell}{\Vert \rvw_\ell \Vert }}{\frac{\rvwh_\ell}{\Vert \rvwh_\ell \Vert}} = \cos(\rtheta_\ell)$. Then, 
% \begin{equation}
% \rvwh_\ell=  \Vert \rvwh_\ell  \Vert \cdot \rmU(\rtheta_\ell) \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
%     \label{eq: quantization to rotation}
% \end{equation}
% where  $\rmU(\rtheta_\ell) \in O(n_\ell)$ is  an orthogonal transformation corresponding to the rotation by $\rtheta_\ell$ in the plane generated by $\rvw_\ell$ and  $\rvwh_\ell$.
% \end{model}
% %can be also represented by a surrogate model, in which  the rotation from $\rvw_\ell$ to  $\rvwh_\ell$ by an angle $\rtheta_\ell$ is represented by an orthogonal transformation $\rmU(\rtheta_\ell) \in O(n_\ell)$. In particular,
% %\begin{equation}
% %\rvwh_\ell=  \Vert \rvwh_\ell  \Vert \cdot \rmU(\rtheta_\ell) \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
% %    \label{eq: quantization to rotation}
% %\end{equation}
% Namely, in this model, the unit vector $\rvw_\ell/\Vert \rvw_\ell \Vert$ is rotated by $\rmU(\rtheta_\ell)$ until it is aligned with the direction of $\rvwh_\ell$, and finally, stretched into the length $\Vert\rvwh_\ell\Vert$.
% Note that $\rtheta_\ell$ is a function of both $\rvw_\ell$ and $\rvwh_\ell$, and thus, for random $\rvw_\ell$ and $\rvwh_\ell$, the resulting $\rtheta_\ell$ is a random variable. 


% Clearly, every point in $\mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell})$ can be attained by \cref{eq: quantization to rotation}. However, knowing $\Vert \rvwh_\ell \Vert, \rtheta_\ell$ and $\rvw_\ell$ is insufficient to determine $\rvwh_\ell$. Specifically, these variables correspond with all vectors $\tilde{\rvw}_\ell$ that reside on a cone that is $\rtheta_\ell$  away from $\rvw_\ell$, for which only a single $\tilde{\rvw}_\ell$ belongs to the lattice. Namely, the lattice point $\rvwh_\ell$ is the point of intersection between this cone and the subspace generated by $\rvw_\ell$ and $\rvwh_\ell$. Thus, any point on the lattice in \cref{eq: uniform vector quant} can be represented by \cref{eq: quantization to rotation}, yet, the opposite direction is not true in general. In the sequel, we analyze the model in \cref{eq: quantization to rotation} and find its rate-distortion minimizing distribution properties. Then, we reflect our findings into the model \cref{eq: uniform vector quant} to find suitable $\Delta_\ell$. Since \cref{eq: uniform vector quant} is a subset of \cref{eq: quantization to rotation}, this yields a nearly optimal solution. 

%\BB{While the all the quantized vectors according to \cref{eq: reconstruct w} falls on a lattice $\gL(\rvb_1,\cdots\rvb_{n_\ell})$ whose basis vectors are $\rvb_1,\cdots\rvb_{n_\ell}$, where each $\rvb_i \in \R^{n_\ell}$, then the surrogate model is the span of this basis as it is continuous. In the sequel we analyze this model.} %On the other hand, conditioning on any pair of variables determines the third variable immediately.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% prop

\begin{proposition}
Let $\rvw_\ell$ be the weights of layer $\ell$, and let $\rvwh_\ell$ denote the quantized representation of those weights, modeled by \cref{eq: quantization to rotation}. Then,  $\rvwh_\ell$ and \RB{$\rvwh_\ell \big| \rvw_\ell$} have a spherical distribution, and thus, it is rotation-invariant. \BB{In preliminaries give small intro to spherical distribution + rotation invariant property.}
\label{prop: rotation invariance of rvwh}
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifshort
Detailed proof is given in \Cref{sec. proof of prop1}.
\else
\input{sections/proofs/prop1}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Essentially, rotation-invariant means that the distributions of $\rvwh_\ell$ and $\rvwh_\ell \big| \rvw_\ell$ do not change when arbitrary rotations are applied to it.  This property is independent of the distribution of $\rvw_\ell$ and $\rtheta_\ell$ and it holds without any assumption on the quantization error or its distribution. \BB{Doesn't it follow from the fact that $\rvwh$ is a rotation of $\rvw$?} %Interestingly, the rotation-invariant property of $\rvwh_\ell$ does not depend on the distribution of $\rvw_\ell$ nor $\rtheta_\ell$. 
%Note that  this proposition holds without any assumption on the quantization error nor its distribution.
The following theorem further strengthens this statement, showing that rotation-invariant distribution is the minimizing distribution of the rate-distortion problem of NNs.   
\begin{theorem}
%Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprises of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. Then, under cosine distance, the unique minimizing distribution of the rate-distortion function is a single-letter product distribution over the layers, where each term $\ell$ in the product is
Let $\gM(\cdot)$ be a NN model with $L$ layers whose weights are $\rvw_{[1:L]}$, and let $\rvwh_{[1:L]}$ denote the quantized representation of those weights. Then, the unique minimizing distribution $p (\wwh_{[1:L]} \big| \ww_{[1:L]})$ of the rate-distortion function
\begin{equation}
   R(D) = \min_{\stackrel{p\prnt{\wwh_{[1:L]} \big| \ww_{[1:L]}}:}{d(\gM(\rvx), \ghM(\rvx)) \leq D}} I \prnt{\rvw_{[1:L]} ;\rvwh_{[1:L]} } 
    \label{eq: R(D) for NNs}
\end{equation}
is a single-letter product distribution, constructed as the product of the layers’ rotation-invariant distribution.
% is a single-letter product distribution over the layers, where each term $\ell$  is a spherical rotation-invariant distribution.
\label{theorem: prod single rotation-invariant}
\end{theorem}

\ifshort
Due to space limitation, the proof of \Cref{theorem: prod single rotation-invariant} is omitted. The key steps are, however, first showing that the minimizing distribution is product distribution. Then, to consider the average distribution of  $\rtheta_\ell$ over the layers, which bounds the mutual information in \cref{eq: R(D) for NNs}. Finally, to show that this average distribution yields a single-letter (scalar) bound, where each layer follows a rotation-invariant distribution by \Cref{prop: rotation invariance of rvwh}. The detailed proof is given in \Cref{sec. proof of theorem1}.
\else
\input{sections/proofs/theorem1}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{align*}
    
% \end{align*}

% Without loss of generality, let us further assume that the rotation of $\rmU_\ell$ is distributed uniformly on the unit sphere in $\R^{n_\ell}$. Thus, the conditional probability is 
% \begin{align*}
%     p\prnt{\rvwh_\ell \big| \rvw_\ell} &= p\prnt{\left.\left\lceil \frac{\rvw_\ell}{\Delta_\ell}\right\rfloor \cdot \Delta_\ell \right| \rvw_\ell} &\\
%     & = p\prnt{\left.\Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} \right| \rvw_\ell} & 
%     % & =  p\prnt{\Vert \rvwh_\ell  \Vert \cdot \tilde{\rmU} \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}, \rvw_\ell}
% \end{align*}
% \begin{equation}
%   \rvwh_\ell= \Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
%   \label{eq: rotated w}
% \end{equation}
% This formulation gives a stochastic representation to $\rvwh_\ell \stackrel{d}{=} \rr_\ell \cdot \rvu_\ell^{(n_\ell)}$, where $\rr = \Vert \rvwh_\ell  \Vert$ is the norm of $\rvwh_\ell$, and $\rvu_\ell^{(n_\ell)} = \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$ is a unit vector that is uniformly distributed on the unit sphere in $\R^{n_\ell}$.
% Accordingly, for any realization of  $\rvw_\ell$, the resulting $p \prnt{\rvwh_\ell \big| \rvw_\ell } = p \prnt{\left. \Vert  \rvwh_\ell   \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} \right| \rvw_\ell}$ is distributed uniformly on a sphere surface with radius $\Vert \rvwh_\ell \Vert$ in $\R^{n_\ell}$. In other words, it is spherically symmetric, and hence, $p\prnt{\rvwh_\ell \big| \rvw_\ell}$ is invariant to rotations \cite[Theorem 2.5]{fang2018symmetric}.  Furthermore, by the law of total probability, averaging over all possible $\rvw_\ell$, yields $p(\rvwh_\ell)$ that is also invariant to rotations. \BB{Hence, $p\prnt{\rvwh_{[1:L]} \big| \rvw_{[1:L]}}$ and $p(\rvwh_{[1:L]})$ are also rotation-invariant. }Note that, due to the convexity of the mutual information,  this minimizing distribution is unique  \cite[Theorem 2.7.4]{thomas2006elements}. 

% The connection between \cref{eq: reconstruct w} to \cref{eq: rotated w} is interesting since. 
% $$ \rvwh_\ell= \Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} = \left\lceil \frac{\rvw}{\Delta}\right\rfloor \cdot \Delta$$


% To prove \Cref{theorem: prod single rotation-invariant},  the following lemma is required.

Still, finding the single-letter solution requires revealing  the exact relation between the distortion at the model's output to the distortion at each layer, which is intricate. Thus, instead of formulating this relation, in \Cref{sec. efficient search} we suggest a searching paradigm that finds efficiently the single-letter constant that satisfies the distortion requirement $D$.  Clearly, this implies using a single parameter for quantizing the whole model, while maintaining the rotation-invariant property in each layer. \BB{The last paragraph is the key statement that not explained well. Need to improve the explanation of our jump from RD minimization to some other algorithm of finding single parameter solution. May be change the order, first provide single parameter search algorithm and then show that it optimal in terms of RD.}
%rely  on the single-letter insight and
%Yet, since the cosine distance  is merely a (bounded) rotation, substituting   $D$ by some distortion $D_\ell$ over the layers in \cref{eq: rate distortion for (a)}, overlooking the exact relation between $D$ and $D_\ell$,  still enables to characterize  the \emph{minimizing distribution of the mutual information}. Moreover, noting that the cosine distance is rotation-invariant by definition, as  the angle between vectors does not change when they are rotated together, further hints that the minimizing distribution should also be a rotation-invariant distribution. 


% \subsubsection{A Wrapping Distortion Measure}
% Given a pre-trained model with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, for which a pre-defined  \emph{cosine distance} is achieved at the outputs.  To assess the distance, calibration samples $\brcs{\rvx}$ are sent through the original model and the quantized model, and the  \emph{average cosine distance} is measured. Namely, $ \frac{1}{B}\sum_{i=1}^B \prnt{1-\cos(\gM(\rvx),\ghM(\rvx))}$.In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable.  Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 

% \RB{Note that considering a mixed-bit solution, where each layer is quantized at a different rate and  the distortion is smaller than a pre-defined threshold almost surely, must reflect in as variable length, max distortion problem, which is formulated differently than the typical rate-distortion \cite[Ch. 25.2]{polyanskiy2014lecture}.}

%The next lemma follows directly by \cite[Theorem~1]{isik2022information} and is given here for completeness.

%  \begin{lemma}
% The cosine distance satisfies the following bound.
% $$ (1-\cos(\angle(\rvv,\hat{\rvv} )) \leq \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2\Vert \rvv \Vert^2}$$
% \label{lemma: cos}
% \end{lemma}
% \begin{proof}[Proof of \Cref{lemma: cos}]
% Assuming $\hat{\rvv} = \rvv + \eps_q$, where the quantization error $\eps_q$ is orthogonal to the vector $\rvv$.  Then, $\Vert \hat{\rvv} \Vert = \Vert \rvv + \eps_q \Vert = \Vert \rvv \Vert + \Vert\eps_q\Vert \geq \Vert \rvv \Vert$. Thus, 
% \begin{align*}
%     \Vert \rvv - \hat{\rvv} \Vert^2  & = \Vert \rvv \Vert^2 + \Vert \hat{\rvv} \Vert^2 -2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
%     & \stackrel{(a)}{\geq} 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert - 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
%     & = 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} &\\
%     & \stackrel{(b)}{\geq} 2\Vert \rvv \Vert^2 \prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))}
% \end{align*}
% where (a) follows by the arithmetic-mean geometric-mean inequality. (b) follows since $\Vert \rvv \Vert \leq \Vert \hat{\rvv}\Vert $. Thus, $\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} \leq  \Vert \rvv - \hat{\rvv} \Vert^2  /  2\Vert \rvv \Vert^2$, which completes the proof.
% \end{proof}

% \begin{lemma}
% Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprise of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. The cosine distance out the output satisfies the following bound.
% \begin{equation}
%     (1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) \leq \prnt{\sum_{\ell=1}^L \prnt{1-\cos(\angle(\rvw_\ell, \rvwh_\ell))}}\prnt{ \frac{\Vert \rvx\Vert^2}{\Vert \gM(\rvx) \Vert^2} \prod_{l=1}^L \Vert \rvw_l \Vert^2}.
%     \label{eq. cos to cos sum}
% \end{equation}
% \label{lemma: cos to sum cos}
% \end{lemma}

% \begin{proof}[Proof of \Cref{lemma: cos to sum cos}]
% \fix{TODO} 
% \end{proof}

% Note that the last term in \cref{eq. cos to cos sum}, $\prnt{\frac{\Vert \rvx\Vert^2}{\Vert \gM(\rvx) \Vert^2}\prod_{l=1}^L \Vert \rvw_l \Vert^2}$ is not affected by the rotation shifts nor the quantization. Thus, this term can be excluded  from the wrapping  distortion function. Accordingly, following \Cref{lemma: cos to sum cos}, we can to minimize 
% $$d(\rvw_{[1:L]}, \rvwh_{[1:L]}) =  \sum_{\ell=1}^L (1- \cos(\angle(\rvw_\ell,\rvwh_\ell)))$$.


 \subsection{Rotation-Invariant Quantization}
As discussed above, among all solutions that satisfy the distortion requirement $D$, a single-letter (scalar) product distribution, constructed as the product of the layers’ rotation-invariant distribution achieves the infimum rate. To fulfil these guidelines, let us examine the relation between $\Delta_\ell$ and the resulting distortion $d(\ww_\ell, \wwh_\ell)$  for each layer $\ell$. The following corollary is useful for this purpose. 

% \begin{lemma}
% Let $\rvw_\ell \in \R^{n_\ell}$ be the weights of layer $\ell$ and let $\rvwh_\ell$ be the quantized representation of those weights, quantized with scale $\Delta_\ell$. Then,
% \[
%  \Vert \rvwh_\ell \Vert^2  =  \Vert  \rvw_\ell \Vert^2 + O(\Delta_\ell^2\cdot n_\ell) 
% \]
% \label{lemma: norm to norm with big order}
% \end{lemma}
% \begin{proof}
% The key-idea for proving the lemma is using the strong law of large numbers. Accordingly,
% \begin{align}
%     \vrnt{\Vert \rvw_\ell \Vert^2 - \Vert \rvwh_\ell \Vert^2} &= \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\rw_{\ell,i}}^2 - \vrnt{\hat{\rw}_{\ell,i}}^2}}&\\
%     & = \Delta_\ell^2 \cdot \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}}^2 - \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}^2} }&\\
%     & = \Delta_\ell^2 \cdot \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}} - \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}}\cdot \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}} +  \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}} }}.
% \end{align}
% where the second equality follows by \cref{eq: reconstruct w}. 
% We point out that the left term in the sum is the quantization error, which can be approximated by a uniform random variable in the high-rate regime \cite[Ch. 25]{polyanskiy2014lecture}. Thus, let us denote by $\reps_i \triangleq \prnt{\frac{\rw_{\ell,i}}{\Delta_\ell} - \round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}$, and assume $\reps_i$ is distributed uniformly over the interval $\brkt{-\frac{1}{2}, \frac{1}{2}}$. Moreover, as $ \round{\frac{\rw_{\ell,i}}{\Delta_\ell}} =  \frac{\rw_{\ell,i}}{\Delta_\ell} - \reps_i$,
% \begin{align}
%     \vrnt{\Vert \rvw_\ell \Vert^2 - \Vert \rvwh_\ell \Vert^2} &= 
%     \Delta_\ell^2 \cdot \vrnt{ \sum_{i=1}^{n_\ell} \prnt{\reps_i \cdot \prnt{2\frac{\rw_{\ell,i}}{\Delta_\ell} - \reps_i }}} &\\
%      & = \Delta_\ell^2\cdot n_\ell \cdot \vrnt{\frac{1}{n_\ell} \cdot\prnt{2\sum_{i=1}^{n_\ell} \reps_i  \frac{\rw_{\ell,i}}{\Delta_\ell} - \sum_{i=1}^{n_\ell} \reps_i^2}} \label{eq: slln} &\\
%      &\stackrel{(a)}{=}  \Delta_\ell^2\cdot n_\ell \cdot\vrnt{\prnt{\E\brkt{\reps_i  \frac{\rw_{\ell,i}}{\Delta_\ell}} - \E[\reps_i^2]} + O(1/\sqrt{n_\ell})} &\label{eq: slln2}\\
%      &\stackrel{(b)}{=} \frac{\Delta_\ell^2\cdot n_\ell}{12} + O(1/\sqrt{n_\ell})
% \end{align}
% where (a) follows since the second moment of $\rw_{\ell,i}$ and $\reps_i$ are finite, and hence, the average in \cref{eq: slln} converges almost surely to the mean, where the rate of convergence is of order $O(1/\sqrt{n_\ell})$, by the strong law of large numbers. (b) follows since the error $\reps_i$ is independent of $\rw_{\ell, i}$, and thus, the average of the left term  in \cref{eq: slln2} converges to
% $\E\brkt{\reps_i  \cdot \frac{\rw_{\ell,i}}{\Delta_\ell}} = \E\brkt{\reps_i} \cdot \E\brkt{ \rw_{\ell,i}/ \Delta_\ell } = 0$,
% since $\E\brkt{\reps_i} = 0$. The right term is converges to $\E[\reps_i^2] = \frac{1}{12}$, which is the variance of the uniform distribution. Thus, the lemma follows
% \end{proof}
% Noticeably, when the scale $\Delta_\ell = o(1/\sqrt{n_\ell})$, i.e., is in the little order of $1/\sqrt{n_\ell}$, then $\Vert \rvwh_\ell \Vert^2  =  \Vert  \rvw_\ell \Vert^2 + o(1)$. Of course, this implies a sufficiently high quantization rate. The following lemma utilizes this observation. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}
% Let $\rvw_\ell$  be the weights vector of layer $\ell$, and $\rvwh_\ell$ be the quantized representation of those weights. Assuming $\Vert \rvwh_\ell \Vert = \Vert \rvw_\ell \Vert + o(\Vert \rvw_\ell \Vert)$, the resulting cosine distance is
% \begin{equation}
% \prnt{1-\cos(\rtheta_\ell)} = \frac{\Vert\rvw_\ell - \rvwh_\ell \Vert^2}{2\Vert \rvw_\ell \Vert^2} + o(1),
%     \label{eq: lemma 1}
% \end{equation}
% where $\rtheta_\ell$ is the angle between $\rvw_\ell$ and $\rvwh_\ell$.
% \label{lemma: cos bound}
% \end{lemma}
% \begin{proof}
% Let $\rvw_\ell$ and $\rvwh_\ell$ be a random vector and its quantized representation, respectively. Then,
% $$\Vert \rvw_\ell - \rvwh_\ell \Vert^2 = \Vert \rvw_\ell \Vert^2 + \Vert \rvwh_\ell \Vert^2 - 2\Vert \rvw_\ell \Vert\cdot \Vert \rvwh_\ell \Vert \cos(\rtheta_\ell).$$
% Now, assuming   $\Vert \rvwh_\ell \Vert = \Vert \rvw_\ell \Vert + o(\Vert \rvw_\ell \Vert)$, yields
% \begin{align*}
%   \Vert \rvw_\ell - \rvwh_\ell \Vert^2 &= 2\Vert \rvw_\ell \Vert^2 + o(\Vert \rvw_\ell \Vert^2) - 2\Vert \rvw_\ell \Vert^2 \cos(\rtheta_\ell) + o(\Vert \rvw_\ell \Vert^2)&\\
%   & =  2\Vert \rvw_\ell \Vert^2\cdot\prnt{1- \cos(\rtheta_\ell)} + o(\Vert \rvw_\ell \Vert^2),  
% \end{align*}
% and hence, when  normalizing both sides by $2\Vert \rvw_\ell \Vert^2$, the  \Cref{lemma: cos bound} follows.
% \end{proof}
% % Now we are ready to prove \Cref{theorem: prod single rotation-invariant}.
% \begin{remark}
% \cite[ Theorem~1]{isik2022information}, and in particular the proof steps therein,  is useful for explaining the relation between $d(\gM(\rvx), \ghM(\rvx))$ and $d(\rvw_\ell, \rvwh_\ell)$ of each layer $\ell$. Specifically, together with \Cref{lemma: cos bound}, it is possible to formulate a  wrapping distortion measure as follows. When $\Vert \ghM(\rvx) \Vert^2 = \Vert \gM(\rvx) \Vert^2 + o(\Vert \gM(\rvx) \Vert)$, and thus,
% $$ (1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) = \frac{\Vert \gM(\rvx) - \ghM(\rvx) \Vert^2}{2\Vert \gM(\rvx) \Vert^2} + o(1),$$
% then, by \cite[ Theorem~1]{isik2022information}, this provides
% \begin{equation}
%     \sup_{\Vert \rvx \Vert^2 \leq 1}(1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) \leq \prnt{\sum_{\ell=1}^L \prnt{1 - \cos(\rtheta_\ell)} +o(1)}\prnt{ \frac{\prod_{l=1}^L \Vert \rvw_l \Vert^2}{\Vert \gM(\rvx) \Vert^2} }.
%     \label{eq. cos to cos sum}
% \end{equation}
% \YR{Where you use eq 26?}
% Since the last term in \cref{eq. cos to cos sum}, $\prnt{\frac{\prod_{l=1}^L \Vert \rvw_l \Vert^2}{\Vert \gM(\rvx) \Vert^2}}$ is not affected by the rotation shifts nor the quantization, it can be excluded  from the wrapping  distortion function. Accordingly, it is possible to consider  the following wrapping distortion measure. 
% \begin{equation}
%     d(\rvw_{[1:L]}, \rvwh_{[1:L]}) =  \frac{1}{L}\sum_{\ell=1}^L (1- \cos(\rtheta_\ell)) \leq D.
%     \label{eq: wrapping distorion}
% \end{equation}
% Nevertheless, for our purpose, which is finding the single-letter rotation-invariant solution, this observation may only provide bounds for the searching problem at hand. In the sequel, however, we derive searching bounds that are relatively tighter. 
% \end{remark}
\BB{Maybe it better described by lemma or theorem instead of corollary?}
\begin{corollary}
Let $\eps_\ell \triangleq d(\ww_\ell, \wwh_\ell)$ be the resulting cosine distance of layer $\ell$, then, its corresponding quantization bin-width \ifshort is $ \Delta_\ell = \sqrt{\eps_\ell} \cdot \Vert \ww_\ell \Vert \cdot \sqrt{24/ n_\ell}$. \else $\Delta_\ell$ is given by
\begin{equation}
    \Delta_\ell = \sqrt{\eps_\ell} \cdot \Vert \ww_\ell \Vert \cdot \sqrt{24/ n_\ell} 
    \label{eq: delta cos}
\end{equation}
\fi
\label{coro: delta to eps}
\end{corollary}
%%%%%%%%%%%%%%%%%%%%%%%%
\ifshort
The proof of \Cref{coro: delta to eps} is deferred to \Cref{sec. proof of coro1}.
\else
\input{sections/proofs/coro1}
\fi
% \YR{\\The transition to MAPE error isn't clear. Currently it looks like inverse SNR error.}
The proof of \Cref{coro: delta to eps} may serve as a proxy to other interesting error criteria such as the \emph{Signal to Quantization Noise Ratio} (SQNR), \cite{caffarena2010sqnr}. Clearly, this yields another relation between  $\Delta_\ell$ and $\epsilon_\ell$. Details in the \Cref{sec. relation to other errors}.

\subsubsection{The Bin-Width and Error Perspective}
\BB{RIQ algorithm still not explained here.} For RIQ, it is desired to choose $\Delta_\ell$ that is proportional to the length $\Vert \ww_\ell \Vert$, since the length is invariant to rotations \BB{Rotation invariant is refers to joint distribution of $\rvw$ and $\rvwh$ but not the length, confusion!!!}, fulfilling the guidelines of being indifferent to the orientation of $\ww_\ell$. This can be attained by requiring $\eps_\ell$ to scale as $n_\ell$  in \Cref{coro: delta to eps} \BB{This is a key point. May be build the algorithm around this idea}.
Noticeably, this makes the formulation of \cref{eq: uniform vector quant} closer to the formulation of \cref{eq: quantization to rotation} \BB{Didn't we said that 7 and 8 both describing quantization?}, which is optimized by a single-letter rotation-invariant solution.

Thus, focusing on a set of $\Delta_{[1:L]}$ that are proportional to the set of lengths $\Vert \ww_{[1:L]} \Vert$, while considering a single-letter solution, we choose $\sqrt{\eps_{\ell}} = \frac{1}{k}\sqrt{\frac{n_\ell}{24}}$ \BB{This step is not clear, may be break it into smaller steps} in \Cref{coro: delta to eps}, \emph{where $k$ is the single-letter parameter that is common to all layers, and should be optimized}. Nevertheless, as $k$ gets large, $\Delta_\ell \to 0$. To prevent this, we add a small constant $\teps$ to $\sqrt{\eps_\ell}$, which bounds the values of the smallest $\Delta_\ell$. The resulting bin-width as a function of $k$ is hence \BB{where is k?} \ifshort $\Delta_\ell(k) = \prnt{\sqrt{\eps_\ell} + \teps} \cdot \Vert \ww_\ell \Vert \cdot \sqrt{24/ n_\ell}$, and thus, \else\fi
% \YR{We have to clarify this. Why $\teps \cdot \sqrt{\frac{24  }{n_\ell}}$}
\BB{We need to think of the intuition to the algorithm. Could we find some visualization or plot to present our algorithm?}
\begin{align}
    \Delta_\ell(k) & = \ifshort \Vert \ww_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps \cdot \sqrt{\frac{24  }{n_\ell}}} & \else \prnt{\sqrt{\eps_\ell} + \teps} \cdot \Vert \ww_\ell \Vert \cdot \sqrt{24/ n_\ell}  & \nonumber\\
    & = \prnt{ \frac{1}{k}\sqrt{{n_\ell}/ {24}} + \teps} \cdot \Vert \ww_\ell \Vert \cdot \sqrt{24/ n_\ell}  & \nonumber\\
    & = \Vert \ww_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps \cdot \sqrt{\frac{24  }{n_\ell}}}
    \fi
    \label{eq: scale}
\end{align}

% where $k$ is a parameter that is common to all layers and $\teps$ is some small constant.


% \Cref{coro: delta to eps} hints that $\Delta_\ell$ can be chosen to be proportional to the length $\Vert \rvw_\ell \Vert$ by letting the per layer cosine distance scale as $\sqrt{n_\ell}$. The motivation for focusing on such $\Delta_\ell$ is the fact that length is invariant to rotations. Noticeably, this makes the vector quantization in \cref{eq: uniform vector quant} closer to the surrogate model  in \cref{eq: quantization to rotation}, which is optimized by a single-letter rotation-invariant solution. Thus, focusing on a set of $\Delta_\ell$ that are proportional to the length, while considering a single-letter solution, we choose in \cref{eq: delta cos} $\sqrt{\eps_{\ell}} = \frac{1}{k}\sqrt{\frac{n_\ell}{24}}$, \emph{where $k$ is a parameter that is common to all layers, and should be optimized}. Note that as $k$ gets large, the scale $\Delta_\ell \to 0$. To prevent this from happening, we add a small constant $\teps$ to $\sqrt{\eps_\ell}$, which bounds the values of the smallest $\Delta_\ell$. The resulting scale as a function of $k$ is hence 
% \begin{equation}
%     \Delta_\ell(k) = \frac{\Vert \rvw_\ell \Vert}{k} + \teps \cdot \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}},
%     \label{eq: scale}
% \end{equation}
% where $k$ is a parameter that is common to all layers and $\teps$ is some small constant.
% \YR{Let's move discussion on $\teps$ to different subsection}
\BB{We have to build a clear way to get to \eqref{eq: scale}}

The additional degree of freedom that $\teps$ \BB{confusion between $\teps$ and $\teps_\ell$.} gives is substantial. For example, it facilitates enforcing quantization to $R$ bits  (e.g., $R=8$  bits) for low precision runtime, by setting the limit $k \to \infty$ at
\ifshort
$ \teps_\ell = \frac{\max(\ww_\ell) - \min(\ww_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \ww_\ell \Vert^2 }{n_\ell}}$.
\else
\begin{equation}
    \teps_\ell = \frac{\max(\ww_\ell) - \min(\ww_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \ww_\ell \Vert^2 }{n_\ell}}.
\label{eq:eps_tilda_constrain}
\end{equation}
\fi

\BB{Also here clarify what is the conclusion.}

% $$\teps_\ell = \frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}}$$
If one wishes to minimize the difference between the histogram of $\rvwh_\ell$ and the theoretical probability distribution of $\rvw_\ell$  at the limit $k\to \infty$, then, by the \cite{freedman1981histogram} rule, one may set \ifshort   $\teps_\ell = 2\frac{IQR(\ww_\ell)}{\sqrt[3]{n_\ell}}$, \else
$$\teps_\ell = 2\frac{IQR(\ww_\ell)}{\sqrt[3]{n_\ell}},$$
\fi
where $IQR(\ww_\ell)$ is the inter-quartile range of $\ww_\ell$. %\YR{Is it used in this section?}
For simplicity, we adopt in the sequel a small common constant value $\teps$ to all layers.
\BB{May be we need to decouple presentation of main algorithm from $\teps$. Explain how the algorithm works w/o $\teps$ to simplify presentation than add more complexity.}
In any case, the resulting quantization rate at layer $\ell$ is
$$R_\ell = \log_2\prnt{\frac{\max(\ww_\ell) - \min(\ww_\ell)}{\Delta_\ell(k)}} = \log_2\prnt{\frac{\max(\ww_\ell) - \min(\ww_\ell)}{\frac{\Vert \ww_\ell \Vert}{k} + \teps \cdot \sqrt{\frac{24 \cdot \Vert \ww_\ell \Vert^2 }{n_\ell}}}} \textnormal{[bits/symbol]}.$$
Increasing $k$ until finding a solution that satisfies the requirement $D$, ensures that the rate $R_\ell$ is induced by the largest $\Delta_\ell$ possible, which is substantial in terms of the resulting entropy in \cref{eq: entropy gain}.  Specifically, such quantization reduces  $-\log_2(\Delta_\ell) = -\log_2(\Vert \ww_\ell\Vert) - \log\prnt{\frac{1}{k} + \teps\sqrt{\frac{24}{n_\ell}}}$ [bits/symbol]. \BB{Again need to explain how we arive to this conclusion.} Then, to achieve (asymptotically) the entropy limit,  an entropy (lossless) compression is applied to the quantized data, so the loss originates only from the quantization part. Obviously, after decoding the symbols, they are stored into one of the nominal representations (e.g., fp32, fp16, int8, etc.), which the hardware supports.

We stress that since the length is invariant to rotations, setting a $\Delta_\ell$ that scales as the length yields a rotation-invariant quantization. Namely, a quantization that is independent of the orientation (direction) of $\ww_\ell$.  Typical quantization, on the other hand, relies on the range, $\max(\ww_\ell) - \min(\ww_\ell)$, whose value depends on the direction of $\ww_\ell$, and hence, changes when $\ww_\ell$ is being rotated. \BB{Again here the last paragraph touching the main point of our method. Instead of optimizing $\Delta$ based on range we optimized it based on length. Then we prove that this produce optimal solution in terms of RD.}


% \begin{lemma}
% Assuming $\Vert \rvv \Vert \approx \Vert \hat{\rvv} \Vert$, the cosine distance is 
% $$(1- \cos\prnt{\angle\prnt{\rvv, \hat{\rvv}}}) \approx \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2 \Vert \rvv\Vert^2}$$
% \end{lemma}

% Before introducing our rotation-invariant quantization, let us briefly discuss the typical quantization procedure. 

% \subsubsection{Typical Quantization Revisited}

% As far as we know, the rotations induced by the linear operations of NN has yet to be addressed. These rotations make the optimization intricate, as it affects the quantization parameters of the successive layers. In the mixed-bit solution, typical quantization requires finding for each layer $\ell$: (a) quantization range $\brcs{\min,\max}_\ell$  (b) quantization rate $R_\ell$ (typically an integer). From these quantities, the quantization bin-width is calculated as
% \begin{equation}
%      \Delta_{\ell} = \frac{(\max - \min)_\ell}{2^{R_\ell}-1}
%     \label{eq: typical bin-width}
% \end{equation}

% Nonetheless, the quantization range is sensitive to rotations. A geometrical interpretation, each layer $\ell$ has its own orientation (direction), length and dimension. The layer's weights get rotated (and stretched) by its input $\rvz_{\ell-1}(\rvx)$, and the output of this layer, $\rvz_{\ell}(\rvx)$ rotates the successive layer's weights, and so on and so forth. Accurate rotation angle through the layers is substantial for the model's performance. Hence, the quantization must be appropriate to all the rotation in the calibration set. However, this is intricate, as each input in the data rotates the layer differently, and the quantization must fulfill all these rotations. To illustrate the difficulty, let us consider a simple example and examine how the rotations affect the quantization range. Assuming  a weight vector $\rvw_\ell = (1,0)$. Clearly, in this case the range is $\max - \min = 1$. However, when a given sample   $\rvx$ rotates  in $45^o$ (counter clockwise) $\max - \min = 0$, as the resulting vector is $(1/\sqrt{2}, 1/\sqrt{2})$. Rotating in the opposite direction, on the other hand, will result in range $\max - \min = 2/\sqrt{2} > 1$.    Thus, it is not clear which range should be used, when considering the rotations applied in the successive layers. (see Figure 5).





%In the sequel, we adopt the wrapping distortion function in \cref{eq: wrapping distorion} throughout our analysis. Before diving into details, let us first revisit the scalar uniform quantizer, and in particular, extends its analysis to vectors in order to obtain the connection of the scale $\Delta_\ell$  to the resulting distortion $d(\rvw_\ell,\rvwh_\ell)$ in each layer $\ell$. For notation simplicity, hereafter the resulting distortion is denoted by $d_\ell \triangleq d(\rvw_\ell,\rvwh_\ell)$.

\subsection{Efficient Searching Method}\label{sec. efficient search}
% \YR{If this is the name of our algorithm "Quantization with Nested Giant-Step Baby-Step" it should be presented at the first paragraph following by description.}
In this section, we introduce an efficient searching algorithm for finding the single-letter solution. In each iteration, the algorithm refines the searching range, until reaching the smallest $k$ (up to a small constant).   Even though the search space is reduced to finding a single parameter $k$, without bounds on $k$, it may be a hard task. 

Let $k^*$ be the optimal (smallest) $k$ that satisfies constraint $D$, and let $\ell^*$ be the index of the layer with the largest $n_\ell$ in $\gM$.  We derive the following bounds for $k^*$.
\begin{proposition}
The value $k^*$ satisfies the following bounds: 
$ \frac{\sqrt{n_{\ell^*} / 24}}{(1-\teps)} \leq k^* \leq \frac{\sqrt{n_{\ell^*} / 24}}{(\teps \cdot \sqrt{\teps})}$.
\label{prop. k bounds}
\end{proposition}
\ifshort
The proof is deferred to  \Cref{sec. proof of prop2}.
\else
\input{sections/proofs/prop2}
\fi
To further improve the search time, a nested refinement is utilized. Specifically,
at each stage, only $\sqrt{\vrnt{\Omega(k)}}$ values of $k$ in an ascending order are considered. Once a certain value of $k$ satisfies the distortion requirement $D$, then, this $k$ becomes the new upper limit for the search, and the search region is refined within a smaller region of $k$ to consider, again with only $\sqrt{\vrnt{\Omega(k)}}$ potential values to inspect. This continues repeatedly until the search step is sufficiently small. This enables fast convergence in relatively few iterations. See Algorithm~\ref{alg: rotation inv} for a detailed description.

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[t]
\footnotesize
\caption{The RIQ algorithm}\label{alg: rotation inv}
\KwData{model weights $\ww_{[1:L]}$, distortion requirement $D$, minimum error $\teps$}
\KwResult{quantized weights $\wwh_{[1:L]}$, such that $d(\gM(\rvx), \ghM(\rvx)) \leq D$}
\textbf{Initialize:} $k_{\min} = \frac{\sqrt{n_{\ell^*}/24}}{1- \teps}$ ,  $\qquad k_{\max} = \frac{\sqrt{n_{\ell^*}/24}}{\sqrt{\teps}\cdot\teps}$,
 $\qquad k = k_{\min}$, $\qquad \textnormal{step} = \sqrt{k_{\max} - k_{\min}}$\;
 \While{$k \leq k_{\max}$}{
%   instructions\;
    \For{$\ell = 1, \cdots, L$}{
        $\Delta_\ell = \Vert \ww_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps\cdot\sqrt{\frac{24}{n_\ell}}}$\;
        $\wwh_\ell = \round{\frac{\ww_\ell}{\Delta_\ell}}\cdot \Delta_\ell$ \;
        }
         
  \eIf{$d(\gM(\rvx), \ghM(\rvx)) \leq D$}
  { 
%   instructions1\;
    \eIf{$\textnormal{step} \leq 3$  \Comment*[r]{Stop condition}}
    {compress to $H(\rvwh_{[1:L]})$ with entropy achieving encoder\;}
    {$k_{\max} = k$\;
    $\textnormal{step} = \sqrt{\textnormal{step}}$\;
    $k = k - \textnormal{step}\cdot \left\lfloor \textnormal{step} \right\rfloor$}
%   instructions2\;
  }{
%   instructions3\;
    $k = k + \textnormal{step}$
  }
}
\label{algorithm}
\normalsize
\end{algorithm}

% \begin{figure}
%     \centering
%     \includegraphics{figures/patterns.pdf}
%     \caption{Caption}
%     \label{fig: patterns}
% \end{figure}

% The \verb|algorithm2e| package also provides a \verb|\listofalgorithms| command that works like \verb|\listoffigures|, but for captioned algorithms:

% \listofalgorithms

==> sections/04_method_o.tex <==
\section{Rotation-invariant  Mixed-bit Quantization}\label{sec. frac}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we study an extended rate-distortion problem for NN models and characterize its minimizing distribution. In particular, first, we introduce a surrogate model that describes vector quantization as rotation and scaling to the nearest lattice point. This model indicates that the distribution of the quantized weights  in each layer is a rotation-invariant distribution.  Then, considering the distance in \cref{eq: cosine dist def} for NN models, the surrogate model reveals that the rate-distortion is  minimized by a single-letter (scalar) product distribution, constructed as the product of the layers' rotation-invariant distribution. In words, the NN model's entropy is minimized when the quantization rates are independent of \emph{the orientation} of the weights vectors $\rvw_{\brkt{1:L}}$. Finally, we design RIQ accordingly and suggest an efficient searching method to find this single-letter solution. 
%\YR{I think this paragraph is already exist as part of problem definition. No need to duplicate since we in limited space.}
%Given a pre-trained model $\gM$ with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, $\ghM$, for which the distance between the outputs is small.  To assess this distance, a sample $\rvx$ is sent through the original model and the quantized model, and the  \emph{cosine distance} between the outputs is measured according to \cref{eq: cosine dist def}. 
%In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable. Yet, since the cosine distance is a bounded measure, as we prove in the sequel, it still allows us to characterize the rate-distortion function, and in particular, the properties of the minimizing distribution.     % Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 

\subsection{Rate-Distortion Analysis of NN Models}
%%%%%%%%%%%%%%%%%%%
%\BB{The considered mixed-bit solution, where each layer is quantized at a different rate and the output distortion is smaller than a pre-defined threshold, resembles  the variable length, maximum distortion flavor of the rate-distortion problem \cite[Ch. 25.2]{polyanskiy2014lecture}.} %Accordingly, we state the following theorem. 

Extending \cref{eq: reconstruct w} to NN model quantization, where layer $\ell$ is encoded uniformly, yields
\begin{equation}
    %\hat{\ubar{w}}_\ell= \left\lceil {\ubar{w}_\ell}/{\Delta_\ell}\right\rfloor \cdot \Delta_\ell.
    \rvwh_\ell= \left\lceil \frac{\rvw_\ell}{\Delta_\ell}\right\rfloor \cdot \Delta_\ell, \qquad \forall \ell=1,...,L.
    \label{eq: uniform vector quant}
\end{equation}
\cite{convay1982fast} showed that this structured quantization motivates a multidimensional lattice model,  where the reconstruction points (vectors) $ \rvwh_\ell$ reside on a lattice grid $\Ls(\rvb_1,\cdots,\rvb_{n_\ell}) \triangleq \brcs{\sum_{i=1}^{n_\ell} \zeta_i \rvb_i \vert \zeta_i \in \Z}$, generated by some  basis $\brcs{\rvb_i}_{i=1}^{n_\ell}$, where each $\rvb_i \in \R^{n_\ell}$. 
Choosing the simplest basis of the form $\Delta_\ell \cdot \mathrm{I}_{n_\ell}$, where $\mathrm{I}_{n_\ell}$ is the $n_\ell \times n_\ell$ identity matrix, allows to associate every vector $ \rvwh_\ell$ with a set of integer coefficients $\zeta_i = \round{\frac{w_{\ell,i}}{\Delta_\ell}}$, for $1\leq i \leq  n_\ell$.  Moreover, the span of these basis vectors,     $\mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell}) \triangleq \brcs{\sum_{i=1}^{n_\ell} \zeta_i \rvb_i \vert \zeta_i \in \R}$, is continuous and thus  $\Ls(\rvb_1,\cdots,\rvb_{n_\ell}) \subset \mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell})$. Since this span covers all points in the lattice, we build a surrogate model that depicts the span and analyze it to provide insights on \cref{eq: uniform vector quant}. %and it is easier to analyze. Accordingly, we build a surrogate model  

\begin{model}
Let $\rvw_\ell$ be the weights of layer $\ell$, and $\rvwh_\ell$ denote the quantized representation of those weights. Let $\rtheta_\ell$ be the rotation angle from $\rvw_\ell$ to  $\rvwh_\ell$, such that $\inp{\frac{\rvw_\ell}{\Vert \rvw_\ell \Vert }}{\frac{\rvwh_\ell}{\Vert \rvwh_\ell \Vert}} = \cos(\rtheta_\ell)$. Then, 
\begin{equation}
\rvwh_\ell=  \Vert \rvwh_\ell  \Vert \cdot \rmU(\rtheta_\ell) \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
    \label{eq: quantization to rotation}
\end{equation}
where  $\rmU(\rtheta_\ell) \in O(n_\ell)$ is  an orthogonal transformation corresponding to the rotation by $\rtheta_\ell$ in the plane generated by $\rvw_\ell$ and  $\rvwh_\ell$.
\end{model}
%can be also represented by a surrogate model, in which  the rotation from $\rvw_\ell$ to  $\rvwh_\ell$ by an angle $\rtheta_\ell$ is represented by an orthogonal transformation $\rmU(\rtheta_\ell) \in O(n_\ell)$. In particular,
%\begin{equation}
%\rvwh_\ell=  \Vert \rvwh_\ell  \Vert \cdot \rmU(\rtheta_\ell) \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
%    \label{eq: quantization to rotation}
%\end{equation}
Namely, in this model, the unit vector $\rvw_\ell/\Vert \rvw_\ell \Vert$ is rotated by $\rmU(\rtheta_\ell)$ until it is aligned with the direction of $\rvwh_\ell$, and finally, stretched into the length $\Vert\rvwh_\ell\Vert$.
Note that $\rtheta_\ell$ is a function of both $\rvw_\ell$ and $\rvwh_\ell$, and thus, for random $\rvw_\ell$ and $\rvwh_\ell$, the resulting $\rtheta_\ell$ is a random variable. 

\BB{}

Clearly, every point in $\mathrm{span}(\rvb_1,\cdots,\rvb_{n_\ell})$ can be attained by \cref{eq: quantization to rotation}. However, knowing $\Vert \rvwh_\ell \Vert, \rtheta_\ell$ and $\rvw_\ell$ is insufficient to determine $\rvwh_\ell$. Specifically, these variables correspond with all vectors $\tilde{\rvw}_\ell$ that reside on a cone that is $\rtheta_\ell$  away from $\rvw_\ell$, for which only a single $\tilde{\rvw}_\ell$ belongs to the lattice. Namely, the lattice point $\rvwh_\ell$ is the point of intersection between this cone and the subspace generated by $\rvw_\ell$ and $\rvwh_\ell$. Thus, any point on the lattice in \cref{eq: uniform vector quant} can be represented by \cref{eq: quantization to rotation}, yet, the opposite direction is not true in general. In the sequel, we analyze the model in \cref{eq: quantization to rotation} and find its rate-distortion minimizing distribution properties. Then, we reflect our findings into the model \cref{eq: uniform vector quant} to find suitable $\Delta_\ell$. Since \cref{eq: uniform vector quant} is a subset of \cref{eq: quantization to rotation}, this yields a nearly optimal solution. 

%\BB{While the all the quantized vectors according to \cref{eq: reconstruct w} falls on a lattice $\gL(\rvb_1,\cdots\rvb_{n_\ell})$ whose basis vectors are $\rvb_1,\cdots\rvb_{n_\ell}$, where each $\rvb_i \in \R^{n_\ell}$, then the surrogate model is the span of this basis as it is continuous. In the sequel we analyze this model.} %On the other hand, conditioning on any pair of variables determines the third variable immediately.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% prop

\begin{proposition}
Let $\rvw_\ell$ be the weights of layer $\ell$, and let $\rvwh_\ell$ denote the quantized representation of those weights, modeled by \cref{eq: quantization to rotation}. Then,  $\rvwh_\ell$ and $\rvwh_\ell \big| \rvw_\ell$ have a spherical rotation-invariant distribution.
\label{prop: rotation invariance of rvwh}
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifshort
Detailed proof is given in \Cref{sec. proof of prop1}.
\else
\input{sections/proofs/prop1}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Essentially, rotation-invariant means that the distributions of $\rvwh_\ell$ and $\rvwh_\ell \big| \rvw_\ell$ do not change when arbitrary rotations are applied to it.  This property is independent of the distribution of $\rvw_\ell$ and $\rtheta_\ell$ and it holds without any assumption on the quantization error or its distribution. %Interestingly, the rotation-invariant property of $\rvwh_\ell$ does not depend on the distribution of $\rvw_\ell$ nor $\rtheta_\ell$. 
%Note that  this proposition holds without any assumption on the quantization error nor its distribution.
The following theorem further strengthens this statement, showing that rotation-invariant distribution is the minimizing distribution of the rate-distortion problem of NNs.   
\begin{theorem}
%Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprises of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. Then, under cosine distance, the unique minimizing distribution of the rate-distortion function is a single-letter product distribution over the layers, where each term $\ell$ in the product is
Let $\gM(\cdot)$ be a NN model with $L$ layers whose weights are $\rvw_{[1:L]}$, and let $\rvwh_{[1:L]}$ denote the quantized representation of those weights. Then, the unique minimizing distribution $p (\rvwh_{[1:L]} \big| \rvw_{[1:L]})$ of the rate-distortion function
\begin{equation}
   R(D) = \min_{\stackrel{p\prnt{\rvwh_{[1:L]} \big| \rvw_{[1:L]}}:}{d(\gM(\rvx), \ghM(\rvx)) \leq D}} I \prnt{\rvw_{[1:L]} ;\rvwh_{[1:L]} } 
    \label{eq: R(D) for NNs}
\end{equation}
is a single-letter product distribution, constructed as the product of the layers’ rotation-invariant distribution.
% is a single-letter product distribution over the layers, where each term $\ell$  is a spherical rotation-invariant distribution.
\label{theorem: prod single rotation-invariant}
\end{theorem}

\ifshort
Due to space limitation, the proof of \Cref{theorem: prod single rotation-invariant} is omitted. The key steps are, however, first showing that the minimizing distribution is product distribution. Then, to consider the average distribution of  $\rtheta_\ell$ over the layers, which bounds the mutual information in \cref{eq: R(D) for NNs}. Finally, to show that this average distribution yields a single-letter (scalar) bound, where each layer follows a rotation-invariant distribution by \Cref{prop: rotation invariance of rvwh}. The detailed proof is given in \Cref{sec. proof of theorem1}.
\else
\input{sections/proofs/theorem1}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{align*}
    
% \end{align*}

% Without loss of generality, let us further assume that the rotation of $\rmU_\ell$ is distributed uniformly on the unit sphere in $\R^{n_\ell}$. Thus, the conditional probability is 
% \begin{align*}
%     p\prnt{\rvwh_\ell \big| \rvw_\ell} &= p\prnt{\left.\left\lceil \frac{\rvw_\ell}{\Delta_\ell}\right\rfloor \cdot \Delta_\ell \right| \rvw_\ell} &\\
%     & = p\prnt{\left.\Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} \right| \rvw_\ell} & 
%     % & =  p\prnt{\Vert \rvwh_\ell  \Vert \cdot \tilde{\rmU} \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}, \rvw_\ell}
% \end{align*}
% \begin{equation}
%   \rvwh_\ell= \Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}.
%   \label{eq: rotated w}
% \end{equation}
% This formulation gives a stochastic representation to $\rvwh_\ell \stackrel{d}{=} \rr_\ell \cdot \rvu_\ell^{(n_\ell)}$, where $\rr = \Vert \rvwh_\ell  \Vert$ is the norm of $\rvwh_\ell$, and $\rvu_\ell^{(n_\ell)} = \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$ is a unit vector that is uniformly distributed on the unit sphere in $\R^{n_\ell}$.
% Accordingly, for any realization of  $\rvw_\ell$, the resulting $p \prnt{\rvwh_\ell \big| \rvw_\ell } = p \prnt{\left. \Vert  \rvwh_\ell   \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} \right| \rvw_\ell}$ is distributed uniformly on a sphere surface with radius $\Vert \rvwh_\ell \Vert$ in $\R^{n_\ell}$. In other words, it is spherically symmetric, and hence, $p\prnt{\rvwh_\ell \big| \rvw_\ell}$ is invariant to rotations \cite[Theorem 2.5]{fang2018symmetric}.  Furthermore, by the law of total probability, averaging over all possible $\rvw_\ell$, yields $p(\rvwh_\ell)$ that is also invariant to rotations. \BB{Hence, $p\prnt{\rvwh_{[1:L]} \big| \rvw_{[1:L]}}$ and $p(\rvwh_{[1:L]})$ are also rotation-invariant. }Note that, due to the convexity of the mutual information,  this minimizing distribution is unique  \cite[Theorem 2.7.4]{thomas2006elements}. 

% The connection between \cref{eq: reconstruct w} to \cref{eq: rotated w} is interesting since. 
% $$ \rvwh_\ell= \Vert \rvwh_\ell  \Vert \cdot \rmU_\ell \cdot \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} = \left\lceil \frac{\rvw}{\Delta}\right\rfloor \cdot \Delta$$


% To prove \Cref{theorem: prod single rotation-invariant},  the following lemma is required.

Still, finding the single-letter solution requires revealing  the exact relation between the distortion at the model's output to the distortion at each layer, which is intricate. Thus, instead of formulating this relation, in \Cref{sec. efficient search} we suggest a searching paradigm that finds efficiently the single-letter constant that satisfies the distortion requirement $D$.  Clearly, this implies using a single parameter for quantizing the whole model, while maintaining the rotation-invariant property in each layer.
%rely  on the single-letter insight and
%Yet, since the cosine distance  is merely a (bounded) rotation, substituting   $D$ by some distortion $D_\ell$ over the layers in \cref{eq: rate distortion for (a)}, overlooking the exact relation between $D$ and $D_\ell$,  still enables to characterize  the \emph{minimizing distribution of the mutual information}. Moreover, noting that the cosine distance is rotation-invariant by definition, as  the angle between vectors does not change when they are rotated together, further hints that the minimizing distribution should also be a rotation-invariant distribution. 


% \subsubsection{A Wrapping Distortion Measure}
% Given a pre-trained model with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, for which a pre-defined  \emph{cosine distance} is achieved at the outputs.  To assess the distance, calibration samples $\brcs{\rvx}$ are sent through the original model and the quantized model, and the  \emph{average cosine distance} is measured. Namely, $ \frac{1}{B}\sum_{i=1}^B \prnt{1-\cos(\gM(\rvx),\ghM(\rvx))}$.In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable.  Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 

% \RB{Note that considering a mixed-bit solution, where each layer is quantized at a different rate and  the distortion is smaller than a pre-defined threshold almost surely, must reflect in as variable length, max distortion problem, which is formulated differently than the typical rate-distortion \cite[Ch. 25.2]{polyanskiy2014lecture}.}

%The next lemma follows directly by \cite[Theorem~1]{isik2022information} and is given here for completeness.

%  \begin{lemma}
% The cosine distance satisfies the following bound.
% $$ (1-\cos(\angle(\rvv,\hat{\rvv} )) \leq \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2\Vert \rvv \Vert^2}$$
% \label{lemma: cos}
% \end{lemma}
% \begin{proof}[Proof of \Cref{lemma: cos}]
% Assuming $\hat{\rvv} = \rvv + \eps_q$, where the quantization error $\eps_q$ is orthogonal to the vector $\rvv$.  Then, $\Vert \hat{\rvv} \Vert = \Vert \rvv + \eps_q \Vert = \Vert \rvv \Vert + \Vert\eps_q\Vert \geq \Vert \rvv \Vert$. Thus, 
% \begin{align*}
%     \Vert \rvv - \hat{\rvv} \Vert^2  & = \Vert \rvv \Vert^2 + \Vert \hat{\rvv} \Vert^2 -2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
%     & \stackrel{(a)}{\geq} 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert - 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
%     & = 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} &\\
%     & \stackrel{(b)}{\geq} 2\Vert \rvv \Vert^2 \prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))}
% \end{align*}
% where (a) follows by the arithmetic-mean geometric-mean inequality. (b) follows since $\Vert \rvv \Vert \leq \Vert \hat{\rvv}\Vert $. Thus, $\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} \leq  \Vert \rvv - \hat{\rvv} \Vert^2  /  2\Vert \rvv \Vert^2$, which completes the proof.
% \end{proof}

% \begin{lemma}
% Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprise of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. The cosine distance out the output satisfies the following bound.
% \begin{equation}
%     (1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) \leq \prnt{\sum_{\ell=1}^L \prnt{1-\cos(\angle(\rvw_\ell, \rvwh_\ell))}}\prnt{ \frac{\Vert \rvx\Vert^2}{\Vert \gM(\rvx) \Vert^2} \prod_{l=1}^L \Vert \rvw_l \Vert^2}.
%     \label{eq. cos to cos sum}
% \end{equation}
% \label{lemma: cos to sum cos}
% \end{lemma}

% \begin{proof}[Proof of \Cref{lemma: cos to sum cos}]
% \fix{TODO} 
% \end{proof}

% Note that the last term in \cref{eq. cos to cos sum}, $\prnt{\frac{\Vert \rvx\Vert^2}{\Vert \gM(\rvx) \Vert^2}\prod_{l=1}^L \Vert \rvw_l \Vert^2}$ is not affected by the rotation shifts nor the quantization. Thus, this term can be excluded  from the wrapping  distortion function. Accordingly, following \Cref{lemma: cos to sum cos}, we can to minimize 
% $$d(\rvw_{[1:L]}, \rvwh_{[1:L]}) =  \sum_{\ell=1}^L (1- \cos(\angle(\rvw_\ell,\rvwh_\ell)))$$.


 \subsection{Rotation-Invariant Quantization}
As discussed above, among all solutions that satisfy the distortion requirement $D$, a single-letter (scalar) product distribution, constructed as the product of the layers’ rotation-invariant distribution achieves the infimum rate. To fulfil these guidelines, let us examine the relation between $\Delta_\ell$ and the resulting distortion $d(\rvw_\ell, \rvwh_\ell)$  for each layer $\ell$. The following corollary is useful for this purpose. 

% \begin{lemma}
% Let $\rvw_\ell \in \R^{n_\ell}$ be the weights of layer $\ell$ and let $\rvwh_\ell$ be the quantized representation of those weights, quantized with scale $\Delta_\ell$. Then,
% \[
%  \Vert \rvwh_\ell \Vert^2  =  \Vert  \rvw_\ell \Vert^2 + O(\Delta_\ell^2\cdot n_\ell) 
% \]
% \label{lemma: norm to norm with big order}
% \end{lemma}
% \begin{proof}
% The key-idea for proving the lemma is using the strong law of large numbers. Accordingly,
% \begin{align}
%     \vrnt{\Vert \rvw_\ell \Vert^2 - \Vert \rvwh_\ell \Vert^2} &= \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\rw_{\ell,i}}^2 - \vrnt{\hat{\rw}_{\ell,i}}^2}}&\\
%     & = \Delta_\ell^2 \cdot \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}}^2 - \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}^2} }&\\
%     & = \Delta_\ell^2 \cdot \vrnt{\sum_{i=1}^{n_\ell} \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}} - \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}}\cdot \prnt{\vrnt{\frac{\rw_{\ell,i}}{\Delta_\ell}} +  \vrnt{\round{\frac{\rw_{\ell,i}}{\Delta_\ell}}} }}.
% \end{align}
% where the second equality follows by \cref{eq: reconstruct w}. 
% We point out that the left term in the sum is the quantization error, which can be approximated by a uniform random variable in the high-rate regime \cite[Ch. 25]{polyanskiy2014lecture}. Thus, let us denote by $\reps_i \triangleq \prnt{\frac{\rw_{\ell,i}}{\Delta_\ell} - \round{\frac{\rw_{\ell,i}}{\Delta_\ell}}}$, and assume $\reps_i$ is distributed uniformly over the interval $\brkt{-\frac{1}{2}, \frac{1}{2}}$. Moreover, as $ \round{\frac{\rw_{\ell,i}}{\Delta_\ell}} =  \frac{\rw_{\ell,i}}{\Delta_\ell} - \reps_i$,
% \begin{align}
%     \vrnt{\Vert \rvw_\ell \Vert^2 - \Vert \rvwh_\ell \Vert^2} &= 
%     \Delta_\ell^2 \cdot \vrnt{ \sum_{i=1}^{n_\ell} \prnt{\reps_i \cdot \prnt{2\frac{\rw_{\ell,i}}{\Delta_\ell} - \reps_i }}} &\\
%      & = \Delta_\ell^2\cdot n_\ell \cdot \vrnt{\frac{1}{n_\ell} \cdot\prnt{2\sum_{i=1}^{n_\ell} \reps_i  \frac{\rw_{\ell,i}}{\Delta_\ell} - \sum_{i=1}^{n_\ell} \reps_i^2}} \label{eq: slln} &\\
%      &\stackrel{(a)}{=}  \Delta_\ell^2\cdot n_\ell \cdot\vrnt{\prnt{\E\brkt{\reps_i  \frac{\rw_{\ell,i}}{\Delta_\ell}} - \E[\reps_i^2]} + O(1/\sqrt{n_\ell})} &\label{eq: slln2}\\
%      &\stackrel{(b)}{=} \frac{\Delta_\ell^2\cdot n_\ell}{12} + O(1/\sqrt{n_\ell})
% \end{align}
% where (a) follows since the second moment of $\rw_{\ell,i}$ and $\reps_i$ are finite, and hence, the average in \cref{eq: slln} converges almost surely to the mean, where the rate of convergence is of order $O(1/\sqrt{n_\ell})$, by the strong law of large numbers. (b) follows since the error $\reps_i$ is independent of $\rw_{\ell, i}$, and thus, the average of the left term  in \cref{eq: slln2} converges to
% $\E\brkt{\reps_i  \cdot \frac{\rw_{\ell,i}}{\Delta_\ell}} = \E\brkt{\reps_i} \cdot \E\brkt{ \rw_{\ell,i}/ \Delta_\ell } = 0$,
% since $\E\brkt{\reps_i} = 0$. The right term is converges to $\E[\reps_i^2] = \frac{1}{12}$, which is the variance of the uniform distribution. Thus, the lemma follows
% \end{proof}
% Noticeably, when the scale $\Delta_\ell = o(1/\sqrt{n_\ell})$, i.e., is in the little order of $1/\sqrt{n_\ell}$, then $\Vert \rvwh_\ell \Vert^2  =  \Vert  \rvw_\ell \Vert^2 + o(1)$. Of course, this implies a sufficiently high quantization rate. The following lemma utilizes this observation. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{lemma}
% Let $\rvw_\ell$  be the weights vector of layer $\ell$, and $\rvwh_\ell$ be the quantized representation of those weights. Assuming $\Vert \rvwh_\ell \Vert = \Vert \rvw_\ell \Vert + o(\Vert \rvw_\ell \Vert)$, the resulting cosine distance is
% \begin{equation}
% \prnt{1-\cos(\rtheta_\ell)} = \frac{\Vert\rvw_\ell - \rvwh_\ell \Vert^2}{2\Vert \rvw_\ell \Vert^2} + o(1),
%     \label{eq: lemma 1}
% \end{equation}
% where $\rtheta_\ell$ is the angle between $\rvw_\ell$ and $\rvwh_\ell$.
% \label{lemma: cos bound}
% \end{lemma}
% \begin{proof}
% Let $\rvw_\ell$ and $\rvwh_\ell$ be a random vector and its quantized representation, respectively. Then,
% $$\Vert \rvw_\ell - \rvwh_\ell \Vert^2 = \Vert \rvw_\ell \Vert^2 + \Vert \rvwh_\ell \Vert^2 - 2\Vert \rvw_\ell \Vert\cdot \Vert \rvwh_\ell \Vert \cos(\rtheta_\ell).$$
% Now, assuming   $\Vert \rvwh_\ell \Vert = \Vert \rvw_\ell \Vert + o(\Vert \rvw_\ell \Vert)$, yields
% \begin{align*}
%   \Vert \rvw_\ell - \rvwh_\ell \Vert^2 &= 2\Vert \rvw_\ell \Vert^2 + o(\Vert \rvw_\ell \Vert^2) - 2\Vert \rvw_\ell \Vert^2 \cos(\rtheta_\ell) + o(\Vert \rvw_\ell \Vert^2)&\\
%   & =  2\Vert \rvw_\ell \Vert^2\cdot\prnt{1- \cos(\rtheta_\ell)} + o(\Vert \rvw_\ell \Vert^2),  
% \end{align*}
% and hence, when  normalizing both sides by $2\Vert \rvw_\ell \Vert^2$, the  \Cref{lemma: cos bound} follows.
% \end{proof}
% % Now we are ready to prove \Cref{theorem: prod single rotation-invariant}.
% \begin{remark}
% \cite[ Theorem~1]{isik2022information}, and in particular the proof steps therein,  is useful for explaining the relation between $d(\gM(\rvx), \ghM(\rvx))$ and $d(\rvw_\ell, \rvwh_\ell)$ of each layer $\ell$. Specifically, together with \Cref{lemma: cos bound}, it is possible to formulate a  wrapping distortion measure as follows. When $\Vert \ghM(\rvx) \Vert^2 = \Vert \gM(\rvx) \Vert^2 + o(\Vert \gM(\rvx) \Vert)$, and thus,
% $$ (1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) = \frac{\Vert \gM(\rvx) - \ghM(\rvx) \Vert^2}{2\Vert \gM(\rvx) \Vert^2} + o(1),$$
% then, by \cite[ Theorem~1]{isik2022information}, this provides
% \begin{equation}
%     \sup_{\Vert \rvx \Vert^2 \leq 1}(1-\cos(\angle(\gM(\rvx),\ghM(\rvx) )) \leq \prnt{\sum_{\ell=1}^L \prnt{1 - \cos(\rtheta_\ell)} +o(1)}\prnt{ \frac{\prod_{l=1}^L \Vert \rvw_l \Vert^2}{\Vert \gM(\rvx) \Vert^2} }.
%     \label{eq. cos to cos sum}
% \end{equation}
% \YR{Where you use eq 26?}
% Since the last term in \cref{eq. cos to cos sum}, $\prnt{\frac{\prod_{l=1}^L \Vert \rvw_l \Vert^2}{\Vert \gM(\rvx) \Vert^2}}$ is not affected by the rotation shifts nor the quantization, it can be excluded  from the wrapping  distortion function. Accordingly, it is possible to consider  the following wrapping distortion measure. 
% \begin{equation}
%     d(\rvw_{[1:L]}, \rvwh_{[1:L]}) =  \frac{1}{L}\sum_{\ell=1}^L (1- \cos(\rtheta_\ell)) \leq D.
%     \label{eq: wrapping distorion}
% \end{equation}
% Nevertheless, for our purpose, which is finding the single-letter rotation-invariant solution, this observation may only provide bounds for the searching problem at hand. In the sequel, however, we derive searching bounds that are relatively tighter. 
% \end{remark}
 
\begin{corollary}
Let $\eps_\ell \triangleq d(\rvw_\ell, \rvwh_\ell)$ be the resulting cosine distance of layer $\ell$, then, its corresponding quantization bin-width \ifshort is $ \Delta_\ell = \sqrt{\eps_\ell} \cdot \Vert \rvw_\ell \Vert \cdot \sqrt{24/ n_\ell}$. \else $\Delta_\ell$ is given by
\begin{equation}
    \Delta_\ell = \sqrt{\eps_\ell} \cdot \Vert \rvw_\ell \Vert \cdot \sqrt{24/ n_\ell} 
    \label{eq: delta cos}
\end{equation}
\fi
\label{coro: delta to eps}
\end{corollary}
%%%%%%%%%%%%%%%%%%%%%%%%
\ifshort
The proof of \Cref{coro: delta to eps} is deferred to \Cref{sec. proof of coro1}.
\else
\input{sections/proofs/coro1}
\fi
% \YR{\\The transition to MAPE error isn't clear. Currently it looks like inverse SNR error.}
The proof of \Cref{coro: delta to eps} may serve as a proxy to other interesting error criteria such as the \emph{Signal to Quantization Noise Ratio} (SQNR), \cite{caffarena2010sqnr}. Clearly, this yields another relation between  $\Delta_\ell$ and $\epsilon_\ell$. Details in the \Cref{sec. relation to other errors}.

\subsubsection{The Bin-Width and Error Perspective}
For RIQ, it is desired to choose $\Delta_\ell$ that is proportional to the length $\Vert \rvw_\ell \Vert$, since the length is invariant to rotations, fulfilling the guidelines of being agnostic to the orientation of $\rvw_\ell$. This can be attained by requiring $\eps_\ell$ to scale as $n_\ell$  in \Cref{coro: delta to eps}.
Noticeably, this makes the formulation of \cref{eq: uniform vector quant} closer to the formulation of \cref{eq: quantization to rotation}, which is optimized by a single-letter rotation-invariant solution.

Thus, focusing on a set of $\Delta_{[1:L]}$ that are proportional to the set of lengths $\Vert \rvw_{[1:L]} \Vert$, while considering a single-letter solution, we choose $\sqrt{\eps_{\ell}} = \frac{1}{k}\sqrt{\frac{n_\ell}{24}}$ in \Cref{coro: delta to eps}, \emph{where $k$ is the single-letter parameter that is common to all layers, and should be optimized}. Nevertheless, as $k$ gets large, $\Delta_\ell \to 0$. To prevent this, we add a small constant $\teps$ to $\sqrt{\eps_\ell}$, which bounds the values of the smallest $\Delta_\ell$. The resulting bin-width as a function of $k$ is hence \ifshort $\Delta_\ell(k) = \prnt{\sqrt{\eps_\ell} + \teps} \cdot \Vert \rvw_\ell \Vert \cdot \sqrt{24/ n_\ell}$, and thus, \else\fi
% \YR{We have to clarify this. Why $\teps \cdot \sqrt{\frac{24  }{n_\ell}}$}
\begin{align}
    \Delta_\ell(k) & = \ifshort \Vert \rvw_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps \cdot \sqrt{\frac{24  }{n_\ell}}} & \else \prnt{\sqrt{\eps_\ell} + \teps} \cdot \Vert \rvw_\ell \Vert \cdot \sqrt{24/ n_\ell}  & \nonumber\\
    & = \prnt{ \frac{1}{k}\sqrt{{n_\ell}/ {24}} + \teps} \cdot \Vert \rvw_\ell \Vert \cdot \sqrt{24/ n_\ell}  & \nonumber\\
    & = \Vert \rvw_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps \cdot \sqrt{\frac{24  }{n_\ell}}}
    \fi
    \label{eq: scale}
\end{align}

% where $k$ is a parameter that is common to all layers and $\teps$ is some small constant.


% \Cref{coro: delta to eps} hints that $\Delta_\ell$ can be chosen to be proportional to the length $\Vert \rvw_\ell \Vert$ by letting the per layer cosine distance scale as $\sqrt{n_\ell}$. The motivation for focusing on such $\Delta_\ell$ is the fact that length is invariant to rotations. Noticeably, this makes the vector quantization in \cref{eq: uniform vector quant} closer to the surrogate model  in \cref{eq: quantization to rotation}, which is optimized by a single-letter rotation-invariant solution. Thus, focusing on a set of $\Delta_\ell$ that are proportional to the length, while considering a single-letter solution, we choose in \cref{eq: delta cos} $\sqrt{\eps_{\ell}} = \frac{1}{k}\sqrt{\frac{n_\ell}{24}}$, \emph{where $k$ is a parameter that is common to all layers, and should be optimized}. Note that as $k$ gets large, the scale $\Delta_\ell \to 0$. To prevent this from happening, we add a small constant $\teps$ to $\sqrt{\eps_\ell}$, which bounds the values of the smallest $\Delta_\ell$. The resulting scale as a function of $k$ is hence 
% \begin{equation}
%     \Delta_\ell(k) = \frac{\Vert \rvw_\ell \Vert}{k} + \teps \cdot \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}},
%     \label{eq: scale}
% \end{equation}
% where $k$ is a parameter that is common to all layers and $\teps$ is some small constant.
% \YR{Let's move discussion on $\teps$ to different subsection}
The additional degree of freedom that $\teps$ gives is substantial. For example, it facilitates enforcing quantization to $R$ bits  (e.g., $R=8$  bits) for low precision runtime, by setting the limit $k \to \infty$ at
\ifshort
$ \teps_\ell = \frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}}$.
\else
\begin{equation}
    \teps_\ell = \frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}}.
\label{eq:eps_tilda_constrain}
\end{equation}
\fi

% $$\teps_\ell = \frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{2^R-1} / \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}}$$
If one wishes to minimize the difference between the histogram of $\rvwh_\ell$ and the theoretical probability distribution of $\rvw_\ell$  at the limit $k\to \infty$, then, by the \cite{freedman1981histogram} rule, one may set \ifshort   $\teps_\ell = 2\frac{IQR(\rvw_\ell)}{\sqrt[3]{n_\ell}}$, \else
$$\teps_\ell = 2\frac{IQR(\rvw_\ell)}{\sqrt[3]{n_\ell}},$$
\fi
where $IQR(\rvw_\ell)$ is the inter-quartile range of $\rvw_\ell$. %\YR{Is it used in this section?}
For simplicity, we adopt in the sequel a small common constant value $\teps$ to all layers.

In any case, the resulting quantization rate at layer $\ell$ is
$$R_\ell = \log_2\prnt{\frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{\Delta_\ell(k)}} = \log_2\prnt{\frac{\max(\rvw_\ell) - \min(\rvw_\ell)}{\frac{\Vert \rvw_\ell \Vert}{k} + \teps \cdot \sqrt{\frac{24 \cdot \Vert \rvw_\ell \Vert^2 }{n_\ell}}}} \textnormal{[bits/symbol]}.$$
Increasing $k$ until finding a solution that satisfies the requirement $D$, ensures that the rate $R_\ell$ is induced by the largest $\Delta_\ell$ possible, which is substantial in terms of the resulting entropy in \cref{eq: entropy gain}.  Specifically, such quantization reduces  $-\log_2(\Delta_\ell) = -\log_2(\Vert \rvw_\ell\Vert) - \log\prnt{\frac{1}{k} + \teps\sqrt{\frac{24}{n_\ell}}}$ [bits/symbol]. Then, to achieve (asymptotically) the entropy limit,  an entropy (lossless) compression is applied to the quantized data, so the loss originates only from the quantization part. Obviously, after decoding the symbols, they are stored into one of the nominal representations (e.g., fp32, fp16, int8, etc.), which the hardware supports.

We stress that since the length is invariant to rotations, setting a $\Delta_\ell$ that scales as the length yields a rotation-invariant quantization. Namely, a quantization that is independent of the orientation (direction) of $\rvw_\ell$.  Typical quantization, on the other hand, relies on the range, $\max(\rvw_\ell) - \min(\rvw_\ell)$, whose value depends on the direction of $\rvw_\ell$, and hence, changes when $\rvw_\ell$ is being rotated.


% \begin{lemma}
% Assuming $\Vert \rvv \Vert \approx \Vert \hat{\rvv} \Vert$, the cosine distance is 
% $$(1- \cos\prnt{\angle\prnt{\rvv, \hat{\rvv}}}) \approx \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2 \Vert \rvv\Vert^2}$$
% \end{lemma}

% Before introducing our rotation-invariant quantization, let us briefly discuss the typical quantization procedure. 

% \subsubsection{Typical Quantization Revisited}

% As far as we know, the rotations induced by the linear operations of NN has yet to be addressed. These rotations make the optimization intricate, as it affects the quantization parameters of the successive layers. In the mixed-bit solution, typical quantization requires finding for each layer $\ell$: (a) quantization range $\brcs{\min,\max}_\ell$  (b) quantization rate $R_\ell$ (typically an integer). From these quantities, the quantization bin-width is calculated as
% \begin{equation}
%      \Delta_{\ell} = \frac{(\max - \min)_\ell}{2^{R_\ell}-1}
%     \label{eq: typical bin-width}
% \end{equation}

% Nonetheless, the quantization range is sensitive to rotations. A geometrical interpretation, each layer $\ell$ has its own orientation (direction), length and dimension. The layer's weights get rotated (and stretched) by its input $\rvz_{\ell-1}(\rvx)$, and the output of this layer, $\rvz_{\ell}(\rvx)$ rotates the successive layer's weights, and so on and so forth. Accurate rotation angle through the layers is substantial for the model's performance. Hence, the quantization must be appropriate to all the rotation in the calibration set. However, this is intricate, as each input in the data rotates the layer differently, and the quantization must fulfill all these rotations. To illustrate the difficulty, let us consider a simple example and examine how the rotations affect the quantization range. Assuming  a weight vector $\rvw_\ell = (1,0)$. Clearly, in this case the range is $\max - \min = 1$. However, when a given sample   $\rvx$ rotates  in $45^o$ (counter clockwise) $\max - \min = 0$, as the resulting vector is $(1/\sqrt{2}, 1/\sqrt{2})$. Rotating in the opposite direction, on the other hand, will result in range $\max - \min = 2/\sqrt{2} > 1$.    Thus, it is not clear which range should be used, when considering the rotations applied in the successive layers. (see Figure 5).





%In the sequel, we adopt the wrapping distortion function in \cref{eq: wrapping distorion} throughout our analysis. Before diving into details, let us first revisit the scalar uniform quantizer, and in particular, extends its analysis to vectors in order to obtain the connection of the scale $\Delta_\ell$  to the resulting distortion $d(\rvw_\ell,\rvwh_\ell)$ in each layer $\ell$. For notation simplicity, hereafter the resulting distortion is denoted by $d_\ell \triangleq d(\rvw_\ell,\rvwh_\ell)$.

\subsection{Efficient Searching Method}\label{sec. efficient search}
% \YR{If this is the name of our algorithm "Quantization with Nested Giant-Step Baby-Step" it should be presented at the first paragraph following by description.}
In this section, we introduce an efficient searching algorithm for finding the single-letter solution. In each iteration, the algorithm refines the searching range, until reaching the smallest $k$ (up to a small constant).   Even though the search space is reduced to finding a single parameter $k$, without bounds on $k$, it may be a hard task. 

Let $k^*$ be the optimal (smallest) $k$ that satisfies constraint $D$, and let $\ell^*$ be the index of the layer with the largest $n_\ell$ in $\gM$.  We derive the following bounds for $k^*$.
\begin{proposition}
The value $k^*$ satisfies the following bounds: 
$ \frac{\sqrt{n_{\ell^*} / 24}}{(1-\teps)} \leq k^* \leq \frac{\sqrt{n_{\ell^*} / 24}}{(\teps \cdot \sqrt{\teps})}$.
\label{prop. k bounds}
\end{proposition}
\ifshort
The proof is deferred to  \Cref{sec. proof of prop2}.
\else
\input{sections/proofs/prop2}
\fi
To further improve the search time, a nested refinement is utilized. Specifically,
at each stage, only $\sqrt{\vrnt{\Omega(k)}}$ values of $k$ in an ascending order are considered. Once a certain value of $k$ satisfies the distortion requirement $D$, then, this $k$ becomes the new upper limit for the search, and the search region is refined within a smaller region of $k$ to consider, again with only $\sqrt{\vrnt{\Omega(k)}}$ potential values to inspect. This continues repeatedly until the search step is sufficiently small. This enables fast convergence in relatively few iterations. See Algorithm~\ref{alg: rotation inv} for a detailed description.

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[t]
\footnotesize
\caption{The RIQ algorithm}\label{alg: rotation inv}
\KwData{model weights $\rvw_{[1:L]}$, distortion requirement $D$, minimum error $\teps$}
\KwResult{quantized weights $\rvwh_{[1:L]}$, such that $d(\gM(\rvx), \ghM(\rvx)) \leq D$}
\textbf{Initialize:} $k_{\min} = \frac{\sqrt{n_{\ell^*}/24}}{1- \teps}$ ,  $\qquad k_{\max} = \frac{\sqrt{n_{\ell^*}/24}}{\sqrt{\teps}\cdot\teps}$,
 $\qquad k = k_{\min}$, $\qquad \textnormal{step} = \sqrt{k_{\max} - k_{\min}}$\;
 \While{$k \leq k_{\max}$}{
%   instructions\;
    \For{$\ell = 1, \cdots, L$}{
        $\Delta_\ell = \Vert \rvw_\ell \Vert\cdot \prnt{\frac{1}{k} + \teps\cdot\sqrt{\frac{24}{n_\ell}}}$\;
        $\rvwh_\ell = \round{\frac{\rvw_\ell}{\Delta_\ell}}\cdot \Delta_\ell$ \;
        }
         
  \eIf{$d(\gM(\rvx), \ghM(\rvx)) \leq D$}
  { 
%   instructions1\;
    \eIf{$\textnormal{step} \leq 3$  \Comment*[r]{Stop condition}}
    {compress to $H(\rvwh_{[1:L]})$ with entropy achieving encoder\;}
    {$k_{\max} = k$\;
    $\textnormal{step} = \sqrt{\textnormal{step}}$\;
    $k = k - \textnormal{step}\cdot \left\lfloor \textnormal{step} \right\rfloor$}
%   instructions2\;
  }{
%   instructions3\;
    $k = k + \textnormal{step}$
  }
}
\label{algorithm}
\normalsize
\end{algorithm}

% \begin{figure}
%     \centering
%     \includegraphics{figures/patterns.pdf}
%     \caption{Caption}
%     \label{fig: patterns}
% \end{figure}

% The \verb|algorithm2e| package also provides a \verb|\listofalgorithms| command that works like \verb|\listoffigures|, but for captioned algorithms:

% \listofalgorithms

==> sections/05_results_A.tex <==
\begin{figure*}
\centering
 \subfigure{
 \centering
    \includegraphics[width=0.45\linewidth]{figures/Cos2Distortion.eps}
    % \caption{Cosine distance of the validation dataset as a function of the deviation constraint (on the calibration dataset). Models include VGG (green circles), ResNet-50 (red squares), and ViT (blue diamonds).}
    \label{fig:Cosine2Distortion}
 }
 \hfill
 \subfigure{
 \centering
    \includegraphics[width=0.43\linewidth]{figures/resnet50.eps}
    % \caption{Accuracy vs Compression for ResNet-50 model. RIQ (green) vs. RAP (orange), OCS (red), linear quantization (cyan), and HAQ (purple). HAQ, however, requires training after the quantization.}
    %Accuracy of Compressed ResNet-50 model vs. the inverse compression ratio. The upper (black) curve shows result of RIQ . The other curves are taken from \cite{pmlr-v139-hubara21a}. Our method clearly outperforms other techniques by achieving better compression rate and higher accuracy.}
    \label{fig:resnet50}
 }
 \caption{(a) Cosine distance of the validation dataset as a function of the deviation constraint (on calibration set). Models include VGG (green), ResNet-50 (red), and ViT (blue). (b) Accuracy vs Compression for ResNet-50 model. RIQ (green) vs. RAP (orange), OCS (red), linear quantization (cyan), and HAQ (purple). HAQ, however, requires training.}
\end{figure*}

\subsubsection{Empirical results}
In this section, we evaluate the compression ratio and model accuracy of RIQ with ANS and compare them to relevant baseline results. In all experiments, we use pre-trained models for their relevant tasks. Specifically, for classification tasks we use \ifshort \else AlexNet \citet{krizhevsky2012imagenet},\fi VGG, \citet{simonyan2014very}, ResNet-50, \citet{he2016deep}, and ViT, \citet{dosovitskiy2020image} models, from the torchvision library\footnote{\href{https://pytorch.org/vision/stable/models.html}{\nolinkurl{pytorch.org/vision/stable/models.html}}} on the ImageNet data-set (I1k). For detection tasks, we use YOLOv5, \citet{glenn_jocher_2022_6222936}, from Neural-Magic library~\footnote{\label{NM}\href{https://sparsezoo.neuralmagic.com}{\nolinkurl{sparsezoo.neuralmagic.com}}} on the COCO dataset \citep{10.1007/978-3-319-10602-1_48}. For NLP task, we use the DistilBERT model, \citet{sanh2019distilbert}, on SQuAD  dataset, \citep{rajpurkar2016squad}. Following RIQ,  an ANS encoder encodes each quantized layer to its entropy limit. An efficient implementation of ANS on GPU was demonstrated by \citet{weissenberger2019massively}, reaching impressive decoding rates. Consequently, RIQ facilitates optimizing and compressing models in a few minutes. For reproduction purposes, we provide a Python code of our algorithm as a supplementary material which includes both the quantization phase (RIQ) and compression phase (ANS)\footnote{\href{https://anonymous.4open.science/r/RIQ-6BE0/README.md}{\nolinkurl{anonymous.4open.science/r/RIQ-6BE0}}}. % Additional results are given in \Cref{sec. additional results}. %~\footnote{\url{https://github.com/ehaleva/RIQ}}

To measure the resulting deviation by \cref{eq: cosine dist def} on a validation set as a function of a deviation requirement $D$, we use two types of calibration data: (a) three real images, sampled from the training, and (b) randomly generated data that follows the Gaussian distribution. In \Cref{fig:Cosine2Distortion} we present the deviation measurements on three models: ResNet-50, VGG, and ViT, where the identity line (black-dotted) is given for reference. As we see, even a small calibration set of three images (solid lines) is sufficient to predict the deviation on the validation set.  Further, we see that the randomly generated data may not predict well the resulting deviation on the validation set, leading to either a less compressed model (ResNet-50 and VGG) or a higher deviation (ViT). %Nevertheless, even with the random data,  RIQ  guarantees that the entropy is minimized for the resulting distortion.



In \Cref{fig:resnet50}, we evaluate the effect of RIQ on the accuracy and the inverse compression ratio (i.e., the reciprocal of \cref{eq:cmp_ratio}) for a pre-trained ResNet-50 model. Interestingly, the rate-distortion curve reflects well the accuracy-compression tradeoff. For comparison, we depict the accuracy-compression results of the \emph{Relaxed Advanced Pipeline} (RAP) method, \citet{pmlr-v139-hubara21a}, \emph{Outlier Channel Splitting} (OCS), \citet{zhao2019improving}, and the \emph{Hardware-aware Automated Quantization} (HAQ), \citet{wang2019haq}, which requires further training for fine-tuning. Indeed, RIQ surpasses other post-training quantization methods, yet, falls short compared to HAQ. This is since retraining the quantized model yields a different rate-distortion curve, which is out of the scope of this paper. 

%to calculate the compression rate of the compressed model.
%
%In \Cref{fig:resnet50} we present the accuracy vs. compression rate for a pre-trained ResNet-50 model. For comparison, we show two other compression techniques and their measured accuracy from \cite{pmlr-v139-hubara21a}. One can see that the proposed algorithm is superior in accuracy as well as in compression ratio to these methods. In addition we present also Hardware-Aware Automated Quantization (HAQ) from \cite{wang2019haq} a compression method that requires further fine tuning of the model, i.e., a short retraining. 



% \subsection{Compression Rate and Distortion Results}
% \YR{We put algorithm pseudocode, not necessary to explain it again in words.}
% In the proposed algorithm we use a calibration dataset and measure the cosine distance between the output of the original model and the quantized one. The resulting distance must be smaller than the distortion constraint. This allows us to find the compressing single letter parameter. 

% \YR{} 


% \subsection{Compression Rate and Model Accuracy}
% Here we evaluate the effect of the compression on the accuracy of the model. We use \cref{eq:cmp_ratio} to calculate the compression rate of the compressed model.


% We define the compression rate as the ratio between the sum of weights in the original model, to the sum of the compressed bit stream and it's decoding tables:

% \begin{equation}
%   \nonumber
%   C = \frac{32*\sum_l n_l}{\sum_l \textrm{length(Bit stream) + size(decode table)}},
% \end{equation}
% assuming that the original model is composed of float32 weights.
% Note, that both quantization and compression is performed per layer in the model. This allows to decompress them layer by layer on the executing machine. 
% In Fig. \ref{fig:resnet50} we present the accuracy vs. compression rate for a pre-trained ResNet-50 model. For comparison, we show two other compression techniques and their measured accuracy from \cite{pmlr-v139-hubara21a}. One can see that the proposed algorithm is superior in accuracy as well as in compression ratio to these methods. In addition we present also Hardware-Aware Automated Quantization (HAQ) from \cite{wang2019haq} a compression method that requires further fine tuning of the model, i.e., a short retraining. 

%Note that the optimization target of the compression scheme presented above is a distortion constraint. The measurements in the RIQ curve (black), from right to left, correspond to a distortion rate of 0.001, 0.005, 0.01, 0.02 and 0.03 respectively.



% \begin{figure}[!tb]
%   \centering
%   %\begin{minipage}[b]{0.45\textwidth}
%     \includegraphics[width=0.60\columnwidth]{figures/resnet50.eps}
%   %\end{minipage}
%   \caption{Accuracy of Compressed ResNet-50 model as a function of the inverse compression rate -- 1/C. The black curve shows result of the proposed algorithm. The other curves are taken from \cite{hubara2020improving}. Per compression rate, the proposed algorithm provides a better accuracy.}
%   \label{fig:resnet50}
% \end{figure}

% In table \ref{table:comparison} below we show comparison to other compression methods. This table is similar in format to the table in \cite{zhang2022post}.
% We had to slightly change the optimization target of the proposed algorithm \ref{algorithm} to provide a compressed model based on compression rate rather than a distortion constraint. Then we compared the accuracy of the quantized model to the original one for two models,
% %three models -- AlexNet \cite{krizhevsky2012imagenet}, 
% VGG and ResNet-50. Our method outperforms other techniques, allows for a much better accuracy per compression rate. We emphasize that our quantization method efficiently combined with the ANS compression scheme allows us to achieve SOTA compression rate with minimal accuracy loss.

% We also stress that our goal is to achieve optimal compression storage-wise rather than addressing the runtime with low precision. Despite that, our technique can constrain the number of bits using \cref{eq: scale} and hence can be combined with quantized execution.

% We conclude this section with the note that among post-training quantization methodologies, RIQ produces SOTA results.

% \YR{Sentence isn't clear. Need to reformulate.}We also note the fact that our compressed model cannot run on dedicated 3-bit, or 4-bit hardware since there is no strict limit on the symbol size. Such limit \emph{can} be introduced through the mechanism explained in Sec. XXX but will lead to a slight deterioration in compression rate and/or accuracy.\YR{}
\begin{table*}[ht]
  \centering 
  \scriptsize
  \begin{threeparttable}
    \caption{Comparison of Top-1 accuracy on ImageNet for various baselines.}
  \label{table:comparison}
    \begin{tabular}{c|c|l c c c }
    \specialrule{.2em}{.1em}{.1em} 
    Model & {\small Compression} & Method & Acc. (\%) & Ref. (\%) & Drop (\%)\\
    \specialrule{.2em}{.1em}{.1em}
    \ifshort\else
    \multirow{7}{*}{AlexNet} 
    & \multirow{2}{*}{$\times 10.6$ (3 bits)} &
    GPFQ \cite{zhang2022post} & 54.77 & 56.52 &  1.75 \\
    & & \textbf{RIQ (Ours)} & \textbf{56.22} & \textbf{56.55} &  \textbf{0.33} \\ 
    \cline{2-6}
     &\multirow{3}{*}{$\times 8$ (4 bits)} & OMSE \cite{choukroun2019low} & 55.52 & 56.62 & 1.10 \\
    & & GPFQ \cite{zhang2022post} & 55.51 & 56.52 &  1.01  \\
    & & \textbf{RIQ (Ours)} & \textbf{56.41} & \textbf{56.55} &  \textbf{0.14}  \\
     \cline{2-6}
     & \multirow{2}{*}{5 bits} & GPFQ \cite{zhang2022post}  & 55.94 & 56.52 & 
     0.58 \\
     & & \textbf{RIQ (Ours)} & \textbf{56.45} & \textbf{56.55} & \textbf{0.1} \\ 
    \specialrule{.2em}{.1em}{.1em}
    \fi
    \multirow{8}{*}{VGG-16} 
    & \multirow{2}{*}{$\times 10.6$ (3 bits)} & GPFQ \cite{zhang2022post} \kern-1em & 70.24 & 71.59&  1.35  \\
    & & \textbf{RIQ (Ours)} & \textbf{71.58} & \textbf{71.59} & \textbf{0.01} \\

    \cline{2-6}
     & \multirow{4}{*}{$\times 8$ (4 bits)} & MSE \cite{banner2019post} \kern-1em & 70.50 &  71.60 & 1.10  \\
     & & OMSE \cite{choukroun2019low} \kern-1em & 71.48 & 73.48 & 2.00 \\
    & & GPFQ \cite{zhang2022post} \kern-1em & 70.90 & 71.59 &  0.69  \\
    & & \textbf{RIQ (Ours)} & \textbf{71.55} & \textbf{71.59} & \textbf{0.04} \\
     \cline{2-6}
     & \multirow{2}{*}{$\times 6.4$ (5 bits)} & GPFQ \cite{zhang2022post} \kern-1em & 71.05 & 71.59 &  0.54  \\
     & & \textbf{RIQ (Ours)} & \textbf{71.58} & \textbf{71.59} & \textbf{0.01} \\

    \specialrule{.2em}{.1em}{.1em} 
    \multirow{14}{*}{ResNet-50} 
     & \multirow{3}{*}{$\times 16$ (2 bits)} & SuRP with tuning \cite{isik2022information} \kern-1em  & \textbf{76.4} & \textbf{76.6} & \textbf{0.2}   \\
     % & & DeepCABAC (with pruning) \cite{Wiedemann2020DeepCABAC} & 74.1 & 74.98 &  0.88 \\
     & & \textbf{RIQ (Ours)} &  69.47 & 76.14 &  6.67 \\
     \cline{2-6}
    & \multirow{2}{*}{$\times 10.6$ (3 bits)} & GPFQ \cite{zhang2022post} \kern-1em  & 70.63 & 76.13 & 5.50   \\
     & & \textbf{RIQ (Ours)} &  \textbf{74.76} & \textbf{76.14} &  \textbf{1.38} \\
     \cline{2-6}
     & \multirow{7}{*}{$\times 8$ (4 bits)}  & MSE \cite{banner2019post} \kern-1em &
     73.80 & 76.10 & 2.30 \\
     & & OMSE \cite{choukroun2019low} \kern-1em &
     73.39 & 76.01 & 2.62 \\
     & & AdaRound \cite{nagel2020up} \kern-1em & 75.23 & 76.07 & 0.84 \\
     & & S-AdaQuant \cite{pmlr-v139-hubara21a} \kern-1em & 75.10 & 77.20 & 2.10 \\
     & & BRECQ \cite{li2021brecq} \kern-1em & 76.29 &  77.00 & 0.71  \\
    & & GPFQ \cite{zhang2022post} \kern-1em  & 74.35 & 76.13 & 1.78   \\
     & & \textbf{RIQ (Ours)} &  \textbf{75.61} & \textbf{76.14} &  \textbf{0.53} \\
     \cline{2-6}
     & \multirow{2}{*}{$\times 6.4$ (5 bits)} & GPFQ \cite{zhang2022post} \kern-1em & 75.26 & 76.13 & 0.87  \\
     & & \textbf{RIQ (Ours)} &  \textbf{75.95} & \textbf{76.14} &  \textbf{0.19} \\

    \specialrule{.2em}{.1em}{.1em} 
    \end{tabular}
  \end{threeparttable}
  \normalsize
\end{table*}


% \begin{table*}[ht]
%   \centering 
%   \tiny
%   \begin{threeparttable}
%     \caption{Comparison of Top-1 accuracy on ImageNet for various quantization techniques.}
%   \label{table:comparison}
%     \begin{tabular}{c|c|l c c c }
%     \specialrule{.2em}{.1em}{.1em} 
%     Model & {\small Compression} & \multicolumn{1}{c}{Method} & Quant. Acc. (\%) & Ref. Acc. (\%) & Acc. Drop (\%)\\
%     \specialrule{.2em}{.1em}{.1em}
%     \ifshort\else
%     \multirow{7}{*}{AlexNet} 
%     & \multirow{2}{*}{$\times 10.6$ (3 bits/symbol)} &
%     GPFQ \cite{zhang2022post} & 54.77 & 56.52 &  1.75 \\
%     & & \textbf{RIQ (Ours)} & \textbf{56.22} & \textbf{56.55} &  \textbf{0.33} \\ 
%     \cline{2-6}
%      &\multirow{3}{*}{$\times 8$ (4 bits/symbol)} & OMSE \cite{choukroun2019low} & 55.52 & 56.62 & 1.10 \\
%     & & GPFQ \cite{zhang2022post} & 55.51 & 56.52 &  1.01  \\
%     & & \textbf{RIQ (Ours)} & \textbf{56.41} & \textbf{56.55} &  \textbf{0.14}  \\
%      \cline{2-6}
%      & \multirow{2}{*}{5 bits/symbol} & GPFQ \cite{zhang2022post}  & 55.94 & 56.52 & 
%      0.58 \\
%      & & \textbf{RIQ (Ours)} & \textbf{56.45} & \textbf{56.55} & \textbf{0.1} \\ 
%     \specialrule{.2em}{.1em}{.1em}
%     \fi
%     \multirow{8}{*}{VGG-16} 
%     & \multirow{2}{*}{$\times 10.6$ (3 bits/symbol)} & GPFQ \cite{zhang2022post} & 70.24 & 71.59&  1.35  \\
%     & & \textbf{RIQ (Ours)} & \textbf{71.58} & \textbf{71.59} & \textbf{0.01} \\

%     \cline{2-6}
%      & \multirow{4}{*}{$\times 8$ (4 bits/symbol)} & MSE \cite{banner2019post} & 70.50 &  71.60 & 1.10  \\
%      & & OMSE \cite{choukroun2019low} & 71.48 & 73.48 & 2.00 \\
%     & & GPFQ \cite{zhang2022post} & 70.90 & 71.59 &  0.69  \\
%     & & \textbf{RIQ (Ours)} & \textbf{71.55} & \textbf{71.59} & \textbf{0.04} \\
%      \cline{2-6}
%      & \multirow{2}{*}{$\times 6.4$ (5 bits/symbol)} & GPFQ \cite{zhang2022post} & 71.05 & 71.59 &  0.54  \\
%      & & \textbf{RIQ (Ours)} & \textbf{71.58} & \textbf{71.59} & \textbf{0.01} \\

%     \specialrule{.2em}{.1em}{.1em} 
%     \multirow{14}{*}{ResNet-50} 
%      & \multirow{3}{*}{$\times 16$ (2 bits/symbol)} & SuRP (with pruning+tuning) \cite{isik2022information}  & \textbf{76.4} & \textbf{76.6} & \textbf{0.2}   \\
%      % & & DeepCABAC (with pruning) \cite{Wiedemann2020DeepCABAC} & 74.1 & 74.98 &  0.88 \\
%      & & \textbf{RIQ (Ours)} &  69.47 & 76.14 &  6.67 \\
%      \cline{2-6}
%     & \multirow{2}{*}{$\times 10.6$ (3 bits/symbol)} & GPFQ \cite{zhang2022post}  & 70.63 & 76.13 & 5.50   \\
%      & & \textbf{RIQ (Ours)} &  \textbf{74.76} & \textbf{76.14} &  \textbf{1.38} \\
%      \cline{2-6}
%      & \multirow{7}{*}{$\times 8$ (4 bits/symbol)}  & MSE \cite{banner2019post} &
%      73.80 & 76.10 & 2.30 \\
%      & & OMSE \cite{choukroun2019low} &
%      73.39 & 76.01 & 2.62 \\
%      & & AdaRound \cite{nagel2020up} & 75.23 & 76.07 & 0.84 \\
%      & & S-AdaQuant \cite{pmlr-v139-hubara21a} & 75.10 & 77.20 & 2.10 \\
%      & & BRECQ \cite{li2021brecq} & 76.29 &  77.00 & 0.71  \\
%     & & GPFQ \cite{zhang2022post}  & 74.35 & 76.13 & 1.78   \\
%      & & \textbf{RIQ (Ours)} &  \textbf{75.61} & \textbf{76.14} &  \textbf{0.53} \\
%      \cline{2-6}
%      & \multirow{2}{*}{$\times 6.4$ (5 bits/symbol)} & GPFQ \cite{zhang2022post} & 75.26 & 76.13 & 0.87  \\
%      & & \textbf{RIQ (Ours)} &  \textbf{75.95} & \textbf{76.14} &  \textbf{0.19} \\

%     \specialrule{.2em}{.1em}{.1em} 
%     \end{tabular}
%   \end{threeparttable}
%   \normalsize
% \end{table*}
In \Cref{table:comparison}, we compare RIQ to relevant baseline methods on the VGG-16 and ResNet-50 models. %This table is similar in format to the table in \cite{zhang2022post}.
In this table, we modified RIQ in Algorithm~\ref{alg: rotation inv} to minimize the deviation (accuracy drop) for a given rate requirement. %obtain a stop condition based on the compression ratio rather than a deviation constraint, and then we measured the resulting accuracy of the quantized models. % for the   
%We had to slightly change the optimization target of the proposed algorithm \ref{algorithm} to provide a compressed model based on compression rate rather than a distortion constraint. Then we compared the accuracy of the quantized model to the original one for two models,
%three models -- AlexNet \cite{krizhevsky2012imagenet}, 
Noticeably, RIQ outperforms most of the baselines, as it reaches the entropy limit by the ANS. Applying ANS to other baselines, however, can only degrade their compression since they consider per-channel quantization, for which the encoding table overhead becomes significant. Further, applying ANS to their layers still degrades compression as the number of unique symbols per-layer is much larger than per-channel. Moreover, some baselines quantized both weights and activation to further accelerate the models. The contribution of ANS to RIQ is discussed in the sequel. %\BB{even though it does not perform range clipping. On the other hand,  Moreover, even if we apply ANS on the method in the table should not yield a further reduction of their size. the table presents the entropy limit attained by the ANS encoding, which was not applied to the other baselines. The contribution of ANS is discussed in \Cref{sec. additional results}.} %\BB{as it presents the entropy limit attained by the ANS encoding, which was not applied to the other baselines. The contribution of ANS is discussed in \Cref{sec. additional results}.} %, yielding better accuracy per compression ratio. %We emphasize that our quantization method efficiently combined with the ANS compression scheme allows us to achieve SOTA compression rate with minimal accuracy loss.
%\BB{Even thought, our objective is to optimize the compression ratio  rather than addressing the runtime with low precision technique, note that RIQ facilitates constraining the number of bits using the proper $\teps$ in \cref{eq: scale}.}
%We also stress that our goal is to achieve optimal compression storage-wise rather than addressing the runtime with low precision. Despite that, our technique can constrain the number of bits using \cref{eq: scale} and hence can be combined with quantized execution.
%We conclude this section with the note that among post-training quantization methodologies, RIQ produces SOTA results.
%\BB{For comparison, we used ANS on other quantized models. For example, GPFQ. The compression does not leads to a redcution in model size for the following reasons. The original quantization (e.g., 5 bit quantization) was implemented per channel. So a full layer contains more than 32 unique values. Hence, its entropy larger than 32 values per layer. Alternatively, when applying ANS per channel suffers from encoding table overhead which deteriorates the compression ratio. Accordingly, even though quantization per channel is beneficial in terms of rate distortion, applying  }

% Typical compression ratio and score achieved by RIQ are presented in \Cref{table:typical} for a variety of models and tasks. Note that the deviation does not translate immediately to the drop in each score, as the latter is a task-specific measure. Yet, in general, the scores improve as the deviation decreases. 
% To further assess the potential of RIQ, we evaluate our method on sparse models taken from the Neural-Magic\footref{NM}. Notably, the compression ratio of sparse models is significantly higher. This coincides with the conclusion that pruning is substantial for good compression \citep{isik2022information}.
% \vspace{-\baselineskip}
%These results are presented in \Cref{table:typical}. For reproduction purposes, we provide a Python implementation of our algorithm. %\footnote{https://www.mindspore.cn/lite/en}
% \begin{table*}[ht]
%   \centering 
%   \tiny
%   \begin{threeparttable}
%     \caption{Comparison of Top-1 accuracy on ImageNet for various quantization techniques.}
%   \label{table:comparison}
%     \begin{tabular}{c|c|l c c c }
%     \specialrule{.2em}{.1em}{.1em} 
%     Model & {\small Compression} & \multicolumn{1}{c}{Method} & Quant. Acc. (\%) & Ref. Acc. (\%) & Acc. Drop (\%)\\
%     \specialrule{.2em}{.1em}{.1em}
%     %\ifshort\else
%     \multirow{7}{*}{ViT / I1k} 
%     & \multirow{2}{*}{$\times 10.6$ (3 bits/symbol)} &
%     GPFQ \cite{zhang2022post} & 54.77 & 56.52 &  1.75 \\
%     & & \textbf{RIQ (Ours)} & \textbf{56.22} & \textbf{56.55} &  \textbf{0.33} \\ 
%     \cline{2-6}
%      &\multirow{3}{*}{$\times 8$ (4 bits/symbol)} & OMSE \cite{choukroun2019low} & 55.52 & 56.62 & 1.10 \\
%     & & GPFQ \cite{zhang2022post} & 55.51 & 56.52 &  1.01  \\
%     & & \textbf{RIQ (Ours)} & \textbf{56.41} & \textbf{56.55} &  \textbf{0.14}  \\
%      \cline{2-6}
%      & \multirow{2}{*}{5 bits/symbol} & GPFQ \cite{zhang2022post}  & 55.94 & 56.52 & 
%      0.58 \\
%      & & \textbf{RIQ (Ours)} & \textbf{56.45} & \textbf{56.55} & \textbf{0.1} \\ 
%     \specialrule{.2em}{.1em}{.1em}
%     %\fi
    
%     \specialrule{.2em}{.1em}{.1em} 
%     \end{tabular}
%   \end{threeparttable}
%   \normalsize
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% new table
% \begin{table*}[ht]
% \scriptsize
%   \centering 
%   \caption{Compression and accuracy achieved by RIQ. Models denoted by asterisk ($^\ast$) were pruned during training, before quantization. 
%   % The metric used to evaluate COCO models is mAP@.5, for classification models we used accuracy in \%. The metric used to evaluate SQuAD models is F1
%   }
%   \label{table:typical}
%   \begin{tabular}{ccccccc}
%   \specialrule{.2em}{.1em}{.1em} 
%   Model / Dataset & Metric & Deviation constraint & Compression & Quant.\ Score  & Ref.\ Score &  Drop \\
%   %& &  &  &  & Score & Drop\\
%   \specialrule{.2em}{.1em}{.1em} 
%   % AlexNet / I1k & Top-1 Acc (\%) & x15.72 & 55.9 & 56.55\\
%     VGG  / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times19.4}$ & 71.3 & 71.59  & \textbf{0.29}\\
%   ResNet-50 / I1k & Top-1 Acc (\%) & 0.5\% &  $\mathbf{\times 7.31}$ & 75.88 & 76.14 & \textbf{0.26}\\
%   ViT / I1k  & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 6.98}$  & 81.0 & 81.07 & \textbf{0.07}\\
%   YOLO / COCO  & mAP@.5 & 0.3\% & $\mathbf{\times 8.34}$ & 54.7 & 55.7 & \textbf{1.0}\\
%   DistilBERT / SQuAD & F1 & 0.025\% & $\mathbf{\times 7.96}$ & 85.0 & 85.08 & \textbf{0.08} \\
%   \hline
%   VGG$^\ast$(75\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 52.9}$ & 69.34 & 69.73 & \textbf{0.39} \\
%   ResNet-50$^\ast$(95\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 41.5}$ & 75.72 & 76.14 & \textbf{0.42}\\
%   YOLO$^\ast$(75\%) / COCO & mAP@.5 & 0.3\% & $\mathbf{\times 16.48}$ & 52.6 & 53.5 & \textbf{0.9}\\
%   DistilBERT$^\ast$(58\%) / SQuAD & F1 & 0.025\% & $\mathbf{\times 19.4}$ & 84.70 & 84.92 & \textbf{0.22} \\
% %  \\
% %  VGG$^\ast$ / I1k & Top-1 Acc (\%) & 0.35\% & $\mathbf{\times 53.0}$ & 69.33 & 69.73 & \textbf{0.4} \\
% %  ResNet-50$^\ast$ / I1k & Top-1 Acc (\%) & 0.05\% & $\mathbf{\times 42.4}$ & 75.83 & 76.14 & \textbf{0.31}\\
% %  YOLO$^\ast$ / COCO & mAP@.5 & 0.4\% & $\mathbf{\times 16.76}$ & 52.5 & 53.5 & \textbf{1}\\
% %  DistilBERT$^\ast$ / SQuAD & F1 & 0.01\% & $\mathbf{\times 20.56}$ & 84.52 & 84.92 & \textbf{0.4} \\
%   \specialrule{.2em}{.1em}{.1em} `
%   \end{tabular}
%   \normalsize
% \end{table*}
% \vspace{-\baselineskip}

% \begin{table*}[ht]
% \tiny
%   \centering 
%   \caption{Compression and accuracy achieved by RIQ. Models denoted by asterisk ($^\ast$) were pruned during training, before quantization. 
%   % The metric used to evaluate COCO models is mAP@.5, for classification models we used accuracy in \%. The metric used to evaluate SQuAD models is F1
%   }
%   \label{table:typical}
%   \begin{tabular}{ccccccc}
%   \specialrule{.2em}{.1em}{.1em} 
%   Model / Dataset & Metric & Deviation constraint & Compression ratio & Quant. Score  & FP32 Ref Score & Score Drop \\
%   %& &  &  &  & Score & Drop\\
%   \specialrule{.2em}{.1em}{.1em} 
%   % AlexNet / I1k & Top-1 Acc (\%) & x15.72 & 55.9 & 56.55\\
%   VGG / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times19.4}$ & 71.3 & 71.59  & \textbf{0.29}\\
%   ResNet-50 / I1k & Top-1 Acc (\%) & 0.5\% &  $\mathbf{\times 7.31}$ & 75.88 & 76.14 & \textbf{0.26}\\
%   ViT / I1k  & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 6.98}$  & 81.0 & 81.07 & \textbf{0.07}\\
%   YOLO / COCO  & mAP@.5 & 0.3\% & $\mathbf{\times 8.34}$ & 54.7 & 55.7 & \textbf{1.0}\\
%   DistilBERT / SQuAD & F1 & 0.025\% & $\mathbf{\times 7.96}$ & 85.0 & 85.08 & \textbf{0.08} \\
%   \hline
%   VGG$^\ast$(75\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 52.9}$ & 69.34 & 69.73 & \textbf{0.39} \\
%   ResNet-50$^\ast$(95\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 41.5}$ & 75.72 & 76.14 & \textbf{0.42}\\
%   YOLO$^\ast$(75\%) / COCO & mAP@.5 & 0.3\% & $\mathbf{\times 16.48}$ & 52.6 & 53.5 & \textbf{0.9}\\
%   DistilBERT$^\ast$(58\%) / SQuAD & F1 & 0.025\% & $\mathbf{\times 19.4}$ & 84.70 & 84.92 & \textbf{0.22} \\
% %  \\
% %  VGG$^\ast$ / I1k & Top-1 Acc (\%) & 0.35\% & $\mathbf{\times 53.0}$ & 69.33 & 69.73 & \textbf{0.4} \\
% %  ResNet-50$^\ast$ / I1k & Top-1 Acc (\%) & 0.05\% & $\mathbf{\times 42.4}$ & 75.83 & 76.14 & \textbf{0.31}\\
% %  YOLO$^\ast$ / COCO & mAP@.5 & 0.4\% & $\mathbf{\times 16.76}$ & 52.5 & 53.5 & \textbf{1}\\
% %  DistilBERT$^\ast$ / SQuAD & F1 & 0.01\% & $\mathbf{\times 20.56}$ & 84.52 & 84.92 & \textbf{0.4} \\
%   \specialrule{.2em}{.1em}{.1em} `
%   \end{tabular}
%   \normalsize
% \end{table*}
% \vspace{-\baselineskip}
%\begin{figure}[!tb]
%  \centering
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/Res%Net50_mixed_bit_FQ_CR_vs_ACC.eps}
%    \caption{Put caption here}
%  \end{minipage}
%  \hfill
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/Res%Net50_mixed_bit_FQ.eps}
%    \caption{Put caption}
%  \end{minipage}
%\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/ResNet-50_mixed_bit_FQ_CR_vs_ACC.eps}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/ResNet-50_mixed_bit_FQ.eps}
%     \caption{Caption}
%     \label{fig:my_label2}
% \end{figure}
%\begin{figure}[!tb]
%  \centering
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/qNE%HVI_video_edit_vignet.eps}%qNEHVI best 13.42  9.9534e-01 %error scaling 10 trials 30_x_4 model %ml_video_edit_vignet.eps}
%    \caption{Put caption here}
%  \end{minipage}
%  \hfill
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/qNE%HVI_best_video_edit_judge.eps}%qNEHVI_best12.61 %9.9986e-01 error scaling 10 trials 30_x_4 model %ml_video_edit_judge.eps}
%    \caption{Put caption}
%  \end{minipage}
%\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/qNEHVI_video_edit_vignet.eps}%qNEHVI best 13.42  9.9534e-01 error scaling 10 trials 30_x_4 model ml_video_edit_vignet.eps}
%     \caption{Caption}
%     \label{fig:my_label3}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/qNEHVI_best_video_edit_judge.eps}%qNEHVI_best12.61 9.9986e-01 error scaling 10 trials 30_x_4 model ml_video_edit_judge.eps}
%     \caption{Caption}
%     \label{fig:my_label4}
% \end{figure}

==> sections/05_results_R.tex <==

\section{Empirical results}
In this section,  we use pre-trained models to evaluate the compression ratio and model accuracy of RIQ  on various tasks. %Specifically, for classification tasks we use \ifshort \else AlexNet \citet{krizhevsky2012imagenet},\fi VGG, \citet{simonyan2014very}, ResNet-50, \citet{he2016deep}, and ViT, \citet{dosovitskiy2020image} models, from the torchvision library\footnote{\href{https://pytorch.org/vision/stable/models.html}{\nolinkurl{pytorch.org/vision/stable/models.html}}} on the ImageNet data-set (I1k). For detection tasks, we use YOLOv5, \citet{glenn_jocher_2022_6222936}, from Neural-Magic library~\footnote{\label{NM}\href{https://sparsezoo.neuralmagic.com}{\nolinkurl{sparsezoo.neuralmagic.com}}} on the COCO dataset \citep{10.1007/978-3-319-10602-1_48}. For NLP task, we use the DistilBERT model, \citet{sanh2019distilbert}, on SQuAD  dataset, \citep{rajpurkar2016squad}.
Following the quantization,  an ANS encoder encodes each quantized layer to its entropy limit. For reproduction purposes, we provide a Python code of our algorithm as a supplementary material\footnote{\href{https://anonymous.4open.science/r/RIQ-6BE0/README.md}{\nolinkurl{anonymous.4open.science/r/RIQ-6BE0}}}. Additional results are given in \Cref{sec. additional results}. %~\footnote{\url{https://github.com/ehaleva/RIQ}}ZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZZ

Typical compression ratio and score achieved by RIQ are presented in \Cref{table:typical} for a variety of models and tasks. Note that the deviation does not translate immediately to the drop in each score, as the latter is a task-specific measure. Yet, in general, the scores improve as the deviation decreases. 
To further assess the potential of RIQ, we evaluate our method on sparse models taken from the Neural-Magic~\footnote{\href{https://sparsezoo.neuralmagic.com}{\nolinkurl{sparsezoo.neuralmagic.com}}}. Notably, the compression ratio of sparse models is significantly higher. This coincides with the conclusion that pruning is substantial for good compression \citep{isik2022information}.
\vspace{-\baselineskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% new table
\begin{table*}[ht]
\scriptsize
  \centering 
  \caption{Compression and accuracy achieved by RIQ. Models denoted by asterisk ($^\ast$) were pruned during training, before quantization. 
  % The metric used to evaluate COCO models is mAP@.5, for classification models we used accuracy in \%. The metric used to evaluate SQuAD models is F1
  }
  \label{table:typical}
  \begin{tabular}{ccccccc}
  \specialrule{.2em}{.1em}{.1em} 
  Model / Dataset & Metric & Deviation constraint & Compression & Quant.\ Score  & Ref.\ Score &  Drop \\
  %& &  &  &  & Score & Drop\\
  \specialrule{.2em}{.1em}{.1em} 
  % AlexNet / I1k & Top-1 Acc (\%) & x15.72 & 55.9 & 56.55\\
    VGG / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times19.4}$ & 71.3 & 71.59  & \textbf{0.29}\\
  ResNet-50 / I1k & Top-1 Acc (\%) & 0.5\% &  $\mathbf{\times 7.31}$ & 75.88 & 76.14 & \textbf{0.26}\\
  ViT / I1k  & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 6.98}$  & 81.0 & 81.07 & \textbf{0.07}\\
  YOLO / COCO  & mAP@.5 & 0.3\% & $\mathbf{\times 8.34}$ & 54.7 & 55.7 & \textbf{1.0}\\
  DistilBERT / SQuAD & F1 & 0.025\% & $\mathbf{\times 7.96}$ & 85.0 & 85.08 & \textbf{0.08} \\
  \hline
  VGG$^\ast$(75\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 52.9}$ & 69.34 & 69.73 & \textbf{0.39} \\
  ResNet-50$^\ast$(95\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 41.5}$ & 75.72 & 76.14 & \textbf{0.42}\\
  YOLO$^\ast$(75\%) / COCO & mAP@.5 & 0.3\% & $\mathbf{\times 16.48}$ & 52.6 & 53.5 & \textbf{0.9}\\
  DistilBERT$^\ast$(58\%) / SQuAD & F1 & 0.025\% & $\mathbf{\times 19.4}$ & 84.70 & 84.92 & \textbf{0.22} \\
%  \\
%  VGG$^\ast$ / I1k & Top-1 Acc (\%) & 0.35\% & $\mathbf{\times 53.0}$ & 69.33 & 69.73 & \textbf{0.4} \\
%  ResNet-50$^\ast$ / I1k & Top-1 Acc (\%) & 0.05\% & $\mathbf{\times 42.4}$ & 75.83 & 76.14 & \textbf{0.31}\\
%  YOLO$^\ast$ / COCO & mAP@.5 & 0.4\% & $\mathbf{\times 16.76}$ & 52.5 & 53.5 & \textbf{1}\\
%  DistilBERT$^\ast$ / SQuAD & F1 & 0.01\% & $\mathbf{\times 20.56}$ & 84.52 & 84.92 & \textbf{0.4} \\
  \specialrule{.2em}{.1em}{.1em} `
  \end{tabular}
  \normalsize
\end{table*}
\vspace{-1.25\baselineskip}

% \begin{table*}[ht]
% \tiny
%   \centering 
%   \caption{Compression and accuracy achieved by RIQ. Models denoted by asterisk ($^\ast$) were pruned during training, before quantization. 
%   % The metric used to evaluate COCO models is mAP@.5, for classification models we used accuracy in \%. The metric used to evaluate SQuAD models is F1
%   }
%   \label{table:typical}
%   \begin{tabular}{ccccccc}
%   \specialrule{.2em}{.1em}{.1em} 
%   Model / Dataset & Metric & Deviation constraint & Compression ratio & Quant. Score  & FP32 Ref Score & Score Drop \\
%   %& &  &  &  & Score & Drop\\
%   \specialrule{.2em}{.1em}{.1em} 
%   % AlexNet / I1k & Top-1 Acc (\%) & x15.72 & 55.9 & 56.55\\
%   VGG / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times19.4}$ & 71.3 & 71.59  & \textbf{0.29}\\
%   ResNet-50 / I1k & Top-1 Acc (\%) & 0.5\% &  $\mathbf{\times 7.31}$ & 75.88 & 76.14 & \textbf{0.26}\\
%   ViT / I1k  & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 6.98}$  & 81.0 & 81.07 & \textbf{0.07}\\
%   YOLO / COCO  & mAP@.5 & 0.3\% & $\mathbf{\times 8.34}$ & 54.7 & 55.7 & \textbf{1.0}\\
%   DistilBERT / SQuAD & F1 & 0.025\% & $\mathbf{\times 7.96}$ & 85.0 & 85.08 & \textbf{0.08} \\
%   \hline
%   VGG$^\ast$(75\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 52.9}$ & 69.34 & 69.73 & \textbf{0.39} \\
%   ResNet-50$^\ast$(95\%) / I1k & Top-1 Acc (\%) & 0.5\% & $\mathbf{\times 41.5}$ & 75.72 & 76.14 & \textbf{0.42}\\
%   YOLO$^\ast$(75\%) / COCO & mAP@.5 & 0.3\% & $\mathbf{\times 16.48}$ & 52.6 & 53.5 & \textbf{0.9}\\
%   DistilBERT$^\ast$(58\%) / SQuAD & F1 & 0.025\% & $\mathbf{\times 19.4}$ & 84.70 & 84.92 & \textbf{0.22} \\
% %  \\
% %  VGG$^\ast$ / I1k & Top-1 Acc (\%) & 0.35\% & $\mathbf{\times 53.0}$ & 69.33 & 69.73 & \textbf{0.4} \\
% %  ResNet-50$^\ast$ / I1k & Top-1 Acc (\%) & 0.05\% & $\mathbf{\times 42.4}$ & 75.83 & 76.14 & \textbf{0.31}\\
% %  YOLO$^\ast$ / COCO & mAP@.5 & 0.4\% & $\mathbf{\times 16.76}$ & 52.5 & 53.5 & \textbf{1}\\
% %  DistilBERT$^\ast$ / SQuAD & F1 & 0.01\% & $\mathbf{\times 20.56}$ & 84.52 & 84.92 & \textbf{0.4} \\
%   \specialrule{.2em}{.1em}{.1em} `
%   \end{tabular}
%   \normalsize
% \end{table*}
% \vspace{-\baselineskip}
%\begin{figure}[!tb]
%  \centering
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/Res%Net50_mixed_bit_FQ_CR_vs_ACC.eps}
%    \caption{Put caption here}
%  \end{minipage}
%  \hfill
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/Res%Net50_mixed_bit_FQ.eps}
%    \caption{Put caption}
%  \end{minipage}
%\end{figure}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/ResNet-50_mixed_bit_FQ_CR_vs_ACC.eps}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/ResNet-50_mixed_bit_FQ.eps}
%     \caption{Caption}
%     \label{fig:my_label2}
% \end{figure}
%\begin{figure}[!tb]
%  \centering
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/qNE%HVI_video_edit_vignet.eps}%qNEHVI best 13.42  9.9534e-01 %error scaling 10 trials 30_x_4 model %ml_video_edit_vignet.eps}
%    \caption{Put caption here}
%  \end{minipage}
%  \hfill
%  \begin{minipage}[b]{0.45\textwidth}
%    \includegraphics[width=0.90\columnwidth]{figures/qNE%HVI_best_video_edit_judge.eps}%qNEHVI_best12.61 %9.9986e-01 error scaling 10 trials 30_x_4 model %ml_video_edit_judge.eps}
%    \caption{Put caption}
%  \end{minipage}
%\end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/qNEHVI_video_edit_vignet.eps}%qNEHVI best 13.42  9.9534e-01 error scaling 10 trials 30_x_4 model ml_video_edit_vignet.eps}
%     \caption{Caption}
%     \label{fig:my_label3}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.40\columnwidth]{figures/qNEHVI_best_video_edit_judge.eps}%qNEHVI_best12.61 9.9986e-01 error scaling 10 trials 30_x_4 model ml_video_edit_judge.eps}
%     \caption{Caption}
%     \label{fig:my_label4}
% \end{figure}

==> sections/_notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}

==> sections/o_frac.tex <==
\section{Fractional Mixed-bit}

In this section we first characterize the distortion measure to be used in the rate-distortion function, for which we derive the  optimal solution characteristics. Then, we  suggest a method that achieves asymptotically this solution. 

Given a pre-trained model with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, for which a pre-defined  \emph{cosine distance} is achieved at the outputs.  To assess the distance, calibration samples $\brcs{\rvx_i}$ are sent through the original model and the quantized model, and the  \emph{average cosine distance} is measured. Namely, $ \frac{1}{B}\sum_{i=1}^B \prnt{1-\cos(\gM(\rvx_i),\ghM(\rvx_i))}$. In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable. Yet, since the cosine distance is a bounded measure, it still allows us to characterize the rate-distortion function, and in particular, the properties of the minimizing distribution.     % Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 



\subsection{Rate-Distortion Function for Model Compression}
%%%%%%%%%%%%%%%%%%%
\RB{When considering a mixed-bit solution, where each layer is quantized at a different rate, and  the distortion at the output is smaller than a pre-defined threshold (almost surely), then, the solution has a form of a variable length, max distortion problem. This solution is  formulated differently than the typical rate-distortion \cite[Ch. 25.2]{polyanskiy2014lecture}}. Accordingly, we state the following theorem. 
\begin{theorem}
Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprises of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. Then, under cosine distance, the unique minimizing rate-distortion distribution is a single-letter product distribution, where each term in the product is a rotation-invariant distribution.
\label{theorem: prod single rotation-invariant}
\end{theorem}
%Let $n_\ell$ denote the number of elements in layer $\ell$, and let $N = \sum_{\ell=1}^L n_\ell$. Then,  given a sample $\rvx_i$, the infimum (achievable) rate $R_i$ required for describing the model's output with expected distortion $D$ is 

 %In words, \cref{eq: R(D|X_i)} is the lowest rate possible for describing the output of the model such that the expected distance at the output is at most $D$
\begin{proof}

Let $d(\rvv, \hat{\rvv}) = 1- \cos\prnt{\angle\prnt{\rvv, \hat{\rvv}}}$ denote the cosine distance between $\rvv$ and $\hat{\rvv}$. Then,  given a sample $\rvx_i$, the infimum (achievable) rate $R_i = R(D | \rvx_i)$ required for describing the model's output with expected distortion $D$ for that sample is 

\begin{align*}
    R(D | \rvx_i)  &= \min_{\stackrel{p\prnt{\hat{\rvw}_{[1:L]} \big| \rvw_{[1:L]},\rvx_i}:}{d(\gM(\rvx_i), \ghM(\rvx_i)) \leq D}} I \prnt{\hat{\rvw}_{[1:L]} ;\rvw_{[1:L]} } &\\
   % &\geq \min_{\stackrel{p\prnt{\hat{\rvw}_{[1:L]} \big| \rvw_{[1:L]},\rvx_i}:}{d(f(\rvx_i), f(\rvx_i)) \leq D}} I \prnt{\hat{\rvw}_{[1:L]} ;\rvw_{[1:L]} } 
    % R_i & = R(D | \rvx_i)  = \min_{\stackrel{p\prnt{\brcs{\hat{\rvw}_\ell}_{\ell=1}^L \big| \brcs{\rvw_\ell}_{\ell=1}^L,\rvx_i}:}{d(\gM(\rvx_i), \ghM(\rvx_i)) \leq D}} I \prnt{\brcs{\hat{\rvw}_\ell}_{\ell=1}^L ;\brcs{\rvw_\ell}_{\ell=1}^L } 
    \label{eq: R(D|X_i)}
\end{align*}
where $p(\hat{\rvw}_{[1:L]} , \rvw_{[1:L]} |\rvx_i) = p(\rvw_{[1:L]} | \rvx_i)p(\hat{\rvw}_{[1:L]} | \rvw_{[1:L]},\rvx_i) $ is the joint probability that satisfies the distortion requirement $D$, and $p(\hat{\rvw}_{[1:L]} | \rvw_{[1:L]},\rvx_i) $ is the distribution that minimizes the mutual information. 

To simplify notation, hereafter we explicitly denote by $I_p(\cdot;\cdot)$ the mutual information under probability $p$. Moreover, we let $\lambda_i = p\prnt{\rvx_i}$ be the probability of $\rvx_i$ for the given calibration set,  and assume  $\sum_i \lambda_i = 1$. Further, we let $\rvz_{\ell-1}(\rvx_i)$ and $\hat{\rvz}_{\ell-1}(\rvx_i)$  be the input of layer $\ell$ at model $\gM$ and $\ghM$ for that sample, respectively. Specifically, for a given sample $\rvx_i$, we denote by $m_\ell(\cdot)$ and $\hat{m}_\ell(\cdot)$ the operators of layer $\ell$, parameterized by $\rvw_\ell$ and $\hat{\rvw}_\ell$, which takes as input $\rvz_{\ell-1}(\rvx_i)$  and $\hat{\rvz}_{\ell-1}(\rvx_i)$ and output $\rvz_{\ell}(\rvx_i)$ and $\hat{\rvz}_{\ell}(\rvx_i)$, respectively. Clearly, this implies $\rvz_0(\rvx_i)= \hat{\rvz}_0(\rvx_i) =\rvx_i$ and that $\rvz_{L}(\rvx_i),\hat{\rvz}_L(\rvx_i)$ are the output of $\gM$ and $\ghM$. 

Note that each sample in the calibration set may yield a different infimum rate $R_i$ for the distortion requirement $D$, and hence, the expected infimum rate for a calibration set $\brcs{\rvx_i}_{i=1}^B$ is
 
\begin{align} 
    R(D) & = \sum_{i=1}^B \lambda_i R(D | \rvx_i) &\\
    & = \sum_{i=1}^B \lambda_i \min_{\stackrel{p\prnt{\hat{\rvw}_{[1:L]} \big| \rvw_{[1:L]},\rvx_i}:}{d(\gM(\rvx_i), \ghM(\rvx_i)) \leq D}} I_{p\prnt{\hat{\rvw}_{[1:L]} \big| \rvw_{[1:L]},\rvx_i}} \prnt{\hat{\rvw}_{[1:L]} ;\rvw_{[1:L]}}  &\\
    & \stackrel{(a)}{=} \sum_{i=1}^B   \lambda_i \sum_{\ell=1}^L \min_{\stackrel{p\prnt{\hat{\rvw}_{\ell} \big| \rvw_{\ell},\rvx_i}:}{d(m_\ell( \rvz_{\ell-1}(\rvx_i)) , \hat{m}_\ell(\hat{\rvz}_{\ell-1}(\rvx_i))) \leq D_\ell}} I_{p(\hat{\rvw}_\ell | \rvw_\ell,\rvx_i)} \prnt{\hat{\rvw}_\ell ; \rvw_\ell } & \label{eq: rate distortion for (a)}\\
     & = \sum_{\ell=1}^L \sum_{i=1}^B  \lambda_i \min_{\stackrel{p\prnt{\hat{\rvw}_{\ell} \big| \rvw_{\ell},\rvx_i}:}{d(m_\ell( \rvz_{\ell-1}(\rvx_i)) , \hat{m}_\ell(\hat{\rvz}_{\ell-1}(\rvx_i))) \leq D_\ell}} I_{p(\hat{\rvw}_\ell | \rvw_\ell,\rvx_i)} \prnt{\hat{\rvw}_\ell ; \rvw_\ell } &\\
     &\stackrel{(b)}{\geq} \sum_{\ell=1}^L  \min_{\stackrel{\sum_{i=1}^B \lambda_i p\prnt{\hat{\rvw}_{\ell} \big| \rvw_{\ell}, \rvx_i}:}{\E_{\sim \lambda}\brkt{d(m_\ell( \rvz_{\ell-1}(\rvx_i)) , \hat{m}_\ell(\hat{\rvz}_{\ell-1}(\rvx_i)))} \leq D_\ell}} I_{\sum_{i=1}^B \lambda_i p(\hat{\rvw}_\ell | \rvw_\ell, \rvx_i)} \prnt{\hat{\rvw}_\ell ; \rvw_\ell } & \label{eq: rate distortion for (b)}  \\
     & =  \sum_{\ell=1}^L  \min_{\stackrel{p\prnt{\hat{\rvw}_{\ell} \big| \rvw_{\ell}}:}{\E_{\sim \lambda}\brkt{d(m_\ell( \rvz_{\ell-1}(\rvx_i)) , \hat{m}_\ell(\hat{\rvz}_{\ell-1}(\rvx_i)))} \leq D_\ell}} I_{p(\hat{\rvw}_\ell | \rvw_\ell)} \prnt{\hat{\rvw}_\ell ; \rvw_\ell } & \label{eq: rate distortion for (c)} & \\
     & = \sum_{\ell=1}^L R_\ell (D_\ell)
     %& =   \min_{\stackrel{p\prnt{\brcs{\hat{\rvw}_\ell}_{\ell=1}^L \big| \brcs{\rvw_\ell}_{\ell=1}^L}:}{\E\brkt{\E_{\sim \lambda}\brkt{d(\gM(\rvx_i) , \hat{\gM}(\rvx_i))}} \leq D}} I_{p\prnt{\brcs{\hat{\rvw}_\ell}_{\ell=1}^L \big| \brcs{\rvw_\ell}_{\ell=1}^L}} \prnt{\brcs{\hat{\rvw}_\ell}_{\ell=1}^L ;\brcs{\rvw_\ell}_{\ell=1}^L } &\\
     %& = R(D | \E_{\sim \lambda}[\rvx_i]) & 
    % \label{eq: rate distortion for set}
\end{align}
where (a) follows %since conditioning reduces entropy. \Cref{eq: rate distortion for (a)}, however, can be achieved with equality
since product distribution minimizes the mutual information \cite[Theorem 5.1, eq. (5.2)]{polyanskiy2014lecture}, and thus, we let $p\prnt{\left. \hat{\rvw}_{[1:L]} \right| \rvw_{[1:L]},\rvx_i} = \prod_{\ell=1}^L p\prnt{\hat{\rvw}_\ell \big| \rvw_\ell ,\rvx_i}$. 
%\RB{Interestingly, the relation between the per layer distortion $D_\ell$ to the output distortion $D$ is derived in \cite[Theorem 1]{isik2022information}, when $\ell_1$-distance is considered. \fix{***sefi: check if we can derive this relation for the cosine similarity, even though it is not a must, it could be nice ***}}  
(b) follows since the mutual information is convex function of the conditional distribution \cite[Theorem 2.7.4]{thomas2006elements}. 

Remarkably, 
%The considered cosine distance is a rotation invariant measure, by definition, as the angle between vectors does not change when both vectors are rotated together. Nevertheless, 
The relation between the distortion at the output to the distortion at each layer is intricate.  Yet, since the cosine distance  is merely a rotation, \cref{eq: rate distortion for (a)} replaces the output rotation distortion $D$ by some rotation distortion $D_\ell$ over the layers. Clearly, the later rotations are always bounded due to the periodicity of the cosine. Thus, even without formulating the exact relation between $D$ and $D_\ell$, knowing that the cosine distance is a bounded measure in each layer, enables us to characterize  the \emph{minimizing distribution of the mutual information}. \BB{In Section~\fix{sec}, we provide a wrapping distortion measure that formalizes this insight by introducing a meaningful bound to the cosine distance at the output.} 

%\BB{cos distance is rotation invariant by definition (angle between vectors does not change when rotated)}

Interestingly, \cref{eq: rate distortion for (b)} provides interesting structure for the optimal mixed-bit solution, as it comprises of the infimum rate in each layer. In particular,
since averaging over the set $\brcs{\rvx_i}$ can only decrease the mutual information in each layer due to convexity, the resulting minimizing distribution of the mutual information $\sum_{i=1}^B \lambda_i p\prnt{\hat{\rvw}_\ell \big| \rvw_\ell, \rvx_i} = p\prnt{\hat{\rvw}_\ell \big| \rvw_\ell}$ is independent of the set $\brcs{\rvx_i}$. %That is, the mutual information in \cref{eq: rate distortion for (b)}, as well as the cosine distance in each layer, are invariant to the rotation of $\rvx_i$. Roughly speaking, each sample $\rvx_i$ rotates eventually all weights $\rvw_\ell$ and $\hat{\rvw}_\ell$ of layers $\ell$, and thus, the optimal quantization should invariant to those rotations of the set $\brcs{\rvx_i}$.  
%This minimizing distribution can be further characterized by noting that the cosine distortion is also rotation invariant, by definition, as the angle between vectors does not change when both vectors are rotated together. In other words, the rotation shifts can be described for each layer independently. 
Moreover, \cref{eq: rate distortion for (b)} implies that each layer should be considered independently.   Let  $\rmU_\ell \in O(n_\ell)$ be a random orthogonal transformation describing the connection (rotation)  between $\hat{\rvw_\ell}$ and $\rvw_\ell$ at each layer $\ell$, such that $\hat{\rvw}_\ell= \Vert \hat{\rvw}_\ell \Vert \rmU_\ell \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$. For a given $\rvw_\ell$, the resulting $\Vert \hat{\rvw}_\ell \Vert \rmU_\ell \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$ is distributed uniformly on a sphere surface with radius $\Vert \hat{\rvw}_\ell \Vert$ in $\R^{n_\ell}$. In other words, it is spherically symmetric, and hence, $p(\hat{\rvw_\ell} \big| \rvw_\ell) \sim p(\Vert \hat{\rvw}_\ell \Vert \rmU_\ell \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} \big| \rvw_\ell) )$ is invariant to rotations \cite[Theorem 2.3]{fang2018symmetric}. Furthermore, by the law of total probability, averaging over all possible $\rvw_\ell$, yields $p(\hat{\rvw}_\ell)$ that is also invariant to rotations. 


%In terms of distortion,  the  cosine distortion is also rotation invariant, by definition, as the angle between vectors does not change when both vectors are rotated together. Consequently, for any orthogonal transformation $\rmU_\ell \in O(n_\ell)$, the minimizing distribution   averaging over many samples (rotations) $\rvx_i$ can only make the mutual information smaller, while the distortion caused by each sample is merely a rotation. Thus, the optimal minimizing distribution is  $p(\hat{\rvw}_\ell | \rvw_\ell)$ which is invariant to rotations. This concludes the proof. 


%The distortion, on the other hand, is a linear function of the distribution $\lambda$ as $ \sum_{i=1}^B \lambda_i D\prnt{p\prnt{\hat{\rvw}_\ell , \rvw_\ell \big| \rvx_i}} = D \prnt{\sum_{i=1}^B \lambda_i p\prnt{\hat{\rvw}_\ell , \rvw_\ell \big| \rvx_i}} $. Hence, the average distortion measured for each sample $\rvx_i$ is equivalent to the distortion caused by the average sample (rotation).
%Moreover, note that cosine distance is rotation invariant by definition as the angle between vectors does not change when both vectors are rotated together. Consequently,  averaging over many samples (rotations) $\rvx_i$ can only make the mutual information smaller, while the distortion caused by each sample is merely a rotation. Thus, the optimal minimizing distribution is  $p(\hat{\rvw}_\ell | \rvw_\ell)$ which is invariant to rotations. This concludes the proof.
%ince only the rotation of each $\rvz^\ell(\rvx_i)$ affects the cosine distance, independently of its norm and independently of the $\rvw_\ell$ norm,  the optimal distribution can be chosen to be rotation invariant. Consequently, the unique rate-distortion achieving must be rotation invariant. Moreover, the optimal solution must quantize each layer independently, since only the product distribution in (a) satisfies the distortion constraint.

\end{proof} 

\subsubsection{A Wrapping Distortion Measure}
% Given a pre-trained model with weight tensors $\rvw_{[1:L]}$, our goal is to obtain the smallest (quantized and compressed) version of this model, for which a pre-defined  \emph{cosine distance} is achieved at the outputs.  To assess the distance, calibration samples $\brcs{\rvx_i}$ are sent through the original model and the quantized model, and the  \emph{average cosine distance} is measured. Namely, $ \frac{1}{B}\sum_{i=1}^B \prnt{1-\cos(\gM(\rvx_i),\ghM(\rvx_i))}$.In the mixed-bit solution, the vital connection between the distortion at the output to the distortion at each layer is intractable.  Instead, we derive an upper bound for the output distortion that involves  distortion in each layer. Inspired by \cite[Theorem~1]{isik2022information}, we formulate the connection between the cosine distance at the output of the models to the cosine distance at each of the layers. 

% \RB{Note that considering a mixed-bit solution, where each layer is quantized at a different rate and  the distortion is smaller than a pre-defined threshold almost surely, must reflect in as variable length, max distortion problem, which is formulated differently than the typical rate-distortion \cite[Ch. 25.2]{polyanskiy2014lecture}.}

%The next lemma follows directly by \cite[Theorem~1]{isik2022information} and is given here for completeness.

 \begin{lemma}
The cosine distance satisfies the following bound.
$$ (1-\cos(\angle(\rvv,\hat{\rvv} )) \leq \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2\Vert \rvv \Vert^2}$$
\label{lemma: cos}
\end{lemma}
\begin{proof}[Proof of \Cref{lemma: cos}]
Assuming $\hat{\rvv} = \rvv + \eps_q$, where the quantization error $\eps_q$ is orthogonal to the vector $\rvv$.  Then, $\Vert \hat{\rvv} \Vert = \Vert \rvv + \eps_q \Vert = \Vert \rvv \Vert + \Vert\eps_q\Vert \geq \Vert \rvv \Vert$. Thus, 
\begin{align*}
    \Vert \rvv - \hat{\rvv} \Vert^2  & = \Vert \rvv \Vert^2 + \Vert \hat{\rvv} \Vert^2 -2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
    & \stackrel{(a)}{\geq} 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert - 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert \cos(\angle(\rvv, \hat{\rvv})) &\\
    & = 2\Vert \rvv \Vert \cdot \Vert \hat{\rvv} \Vert\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} &\\
    & \stackrel{(b)}{\geq} 2\Vert \rvv \Vert^2 \prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))}
\end{align*}
where (a) follows by the arithmetic-mean geometric-mean inequality. (b) follows since $\Vert \rvv \Vert \leq \Vert \hat{\rvv}\Vert $. Thus, $\prnt{1 - \cos(\angle(\rvv, \hat{\rvv}))} \leq  \Vert \rvv - \hat{\rvv} \Vert^2  /  2\Vert \rvv \Vert^2$, which completes the proof.
\end{proof}

\begin{lemma}
Assuming $\gM(\cdot)$ is a NN model with $L$ layers, each comprise of a linear operator and a non-linear $1$-Lipschitz activation $\sigma(\cdot)$. The cosine distance out the output satisfies the following bound.
\begin{equation}
    (1-\cos(\angle(\gM(\rvx_i),\ghM(\rvx_i) )) \leq \prnt{\sum_{\ell=1}^L \prnt{1-\cos(\angle(\rvw_\ell, \hat{\rvw}_\ell))}}\prnt{ \frac{\Vert \rvx_i\Vert^2}{\Vert \gM(\rvx_i) \Vert^2} \prod_{l=1}^L \Vert \rvw_l \Vert^2}.
    \label{eq. cos to cos sum}
\end{equation}
\label{lemma: cos to sum cos}
\end{lemma}

\begin{proof}[Proof of \Cref{lemma: cos to sum cos}]
\fix{TODO} 
\end{proof}

Note that the last term in \cref{eq. cos to cos sum}, $\prnt{\frac{\Vert \rvx_i\Vert^2}{\Vert \gM(\rvx_i) \Vert^2}\prod_{l=1}^L \Vert \rvw_l \Vert^2}$ is not affected by the rotation shifts nor the quantization. Thus, this term can be excluded  from the wrapping  distortion function. Accordingly, following \Cref{lemma: cos to sum cos}, we can to minimize 
$$d(\rvw_{[1:L]}, \hat{\rvw}_{[1:L]}) =  \sum_{\ell=1}^L (1- \cos(\angle(\rvw_\ell,\hat{\rvw}_\ell)))$$.


 \subsection{Rotation-Invariant Quantization}
Before we dive into details, let us first revisit the scalar uniform quantizer, and in particular, extends its analysis to vectors in order to obtain the connection of the bin width $\Delta_\ell$  to the resulting quantization error $\eps_\ell$ of layer $\ell$. When considering a separable distortion like the MSE, the distortion is simply the average of the  form of  \cref{eq. scalar quant}. Thus, by law of large numbers, for layer $\ell$ we have, 
\begin{align}
  \E \Vert \rvw_\ell- \hat{\rvw}_\ell \Vert^2 & = \frac{1}{n_\ell} \sum_{j=1}^{n_\ell} \E \vert \rw_{\ell,j}- \hat{\rw}_{\ell,j} \vert^2  &\nonumber \\
  &\stackrel{(a)}{=} \frac{1}{n_\ell}\sum_{j=1}^{n_\ell} \vert \rw_{\ell,j}- \hat{\rw}_{\ell,j}  \vert^2 + o(1) &\nonumber \\
  &= \frac{1}{n_\ell} \Vert \rvw_\ell - \hat{\rvw}_\ell \Vert^2 + o(1) =   \Delta^2_\ell / 12 + o(1) \label{eq. mse vector quant}
\end{align}
where (a) follows by the law of large numbers. Hereafter we omit the little order $o(1)$ for clarity of notation. 

Interestingly, from the MSE in \cref{eq. mse vector quant} other error criteria can be extracted.
For example, the \emph{Mean Absolute Percentage Error} (MAPE) can be obtained  as follows.
\begin{equation}
  \eps_{rel} \triangleq \frac{\Vert  \rvw_\ell - \hat{ \rvw}_\ell  \Vert }{\Vert \rvw_\ell \Vert } = \sqrt{\frac{\Delta^2_\ell}{12} \cdot \frac{n_\ell}{\Vert \rvw_\ell\Vert^2}}  
\end{equation}
Or, equivalently, 
\begin{equation}
  \Delta_\ell = \eps_{rel} \Vert \rvw_\ell \Vert \sqrt{12/ n_\ell} 
\end{equation}

To derive \emph{cosine distance} criterion, first note that the cosine distance is equivalent to Euclidean distance of normalized vectors up to a constant. Thus, assuming that for each layer $\ell$ the norms $\Vert\hat{\rvw}_\ell \Vert \approx \Vert \rvw_\ell \Vert$ are about the same, we observe $\Vert \rvw_\ell -\hat{\rvw}_\ell \Vert^2 \approx 2\Vert\rvw_\ell\Vert^2(1-\cos(\angle(\rvw_\ell, \hat{\rvw}_\ell))) $. Hence, 

\begin{equation}
  \eps_{\cos} \triangleq (1-\cos(\angle(\rvw_\ell, \hat{\rvw}_\ell))) \approx \frac{\Vert  \rvw_\ell - \hat{ \rvw}_\ell  \Vert^2}{2\Vert \rvw_\ell \Vert^2} =  \frac{\Delta^2_\ell}{24} \cdot \frac{n_\ell}{\Vert \rvw_\ell\Vert^2}  
  \label{eq: eps cos}
\end{equation}
Or, in terms of $\Delta_\ell$, 
\begin{equation}
  \Delta_\ell = \sqrt{\eps_{\cos}} \Vert \rvw_\ell \Vert \sqrt{24/ n_\ell} 
  \label{eq: delta cos}
\end{equation}
Hereafter, for clarity, we focus on the cos distance analysis.

\Cref{eq: eps cos} and \cref{eq: delta cos} hint that we can pick $\Delta_\ell$ that is proportional to $\Vert \rvw_\ell \Vert$ by letting the local quantization errors scale with $n_\ell$. Specifically, setting $\sqrt{\eps_{\cos}(k)} = \frac{1}{k}\sqrt{\frac{n_ell}{24}}$ , where $k$ is a parameter that should be optimized. Yet, as $k$ gets larger the local errors goes to zero, which implies $\Delta_\ell \to 0$. Thus, we restrict $\Delta_\ell$ by adding a small constant $\tilde{\eps}$ that prevents this from happening. Accordingly, for the cosine distance, picking 

\subsection{Efficient Searching Method}


% \begin{lemma}
% Assuming $\Vert \rvv \Vert \approx \Vert \hat{\rvv} \Vert$, the cosine distance is 
% $$(1- \cos\prnt{\angle\prnt{\rvv, \hat{\rvv}}}) \approx \frac{\Vert \rvv - \hat{\rvv} \Vert^2}{2 \Vert \rvv\Vert^2}$$
% \end{lemma}

% Before introducing our rotation-invariant quantization, let us briefly discuss the typical quantization procedure. 

% \subsubsection{Typical Quantization Revisited}

% As far as we know, the rotations induced by the linear operations of NN has yet to be addressed. These rotations make the optimization intricate, as it affects the quantization parameters of the successive layers. In the mixed-bit solution, typical quantization requires finding for each layer $\ell$: (a) quantization range $\brcs{\min,\max}_\ell$  (b) quantization rate $R_\ell$ (typically an integer). From these quantities, the quantization bin-width is calculated as
% \begin{equation}
%      \Delta_{\ell} = \frac{(\max - \min)_\ell}{2^{R_\ell}-1}
%     \label{eq: typical bin-width}
% \end{equation}

% Nonetheless, the quantization range is sensitive to rotations. A geometrical interpretation, each layer $\ell$ has its own orientation (direction), length and dimension. The layer's weights get rotated (and stretched) by its input $\rvz_{\ell-1}(\rvx)$, and the output of this layer, $\rvz_{\ell}(\rvx)$ rotates the successive layer's weights, and so on and so forth. Accurate rotation angle through the layers is substantial for the model's performance. Hence, the quantization must be appropriate to all the rotation in the calibration set. However, this is intricate, as each input in the data rotates the layer differently, and the quantization must fulfill all these rotations. To illustrate the difficulty, let us consider a simple example and examine how the rotations affect the quantization range. Assuming  a weight vector $\rvw_\ell = (1,0)$. Clearly, in this case the range is $\max - \min = 1$. However, when a given sample   $\rvx_i$ rotates  in $45^o$ (counter clockwise) $\max - \min = 0$, as the resulting vector is $(1/\sqrt{2}, 1/\sqrt{2})$. Rotating in the opposite direction, on the other hand, will result in range $\max - \min = 2/\sqrt{2} > 1$.    Thus, it is not clear which range should be used, when considering the rotations applied in the successive layers. (see Figure 5).

==> sections/proofs/prop1_R.tex <==


\begin{itemize}
    \item given w, consider U nxn such that U w is distrubted uniformly on a sphere
    \item the transformation to spherical coordinates
    \item theorem 2.13
\end{itemize}

\begin{proof}
For any given realization of the vector $\rvw_\ell$, consider the unit vector $\rvw_\ell/ \Vert \rvw_\ell \Vert$, and a random orthogonal matrix $\rmU$ with the distribution having the support of the set of $n_\ell \times n_\ell$ orthogonal matrices \citep{Mezzadri2006HowTG}. Then, $\rvu \triangleq \rmU \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$ is distributed uniformly on a sphere $\sS^{n_\ell}$.

Considering the transformation of $\rvu$ to spherical coordinates yields a representation in which the elements of $\rvu$ are independent by \citet[Theorem 2.11]{fang2018symmetric}.

Finally, conditioning over any element in this spherical representation 

uniformly on a sphere

By \cite[Theorem 4.3]{fang2018symmetric}, a necessary and sufficient condition for  $\rvwt_\ell\big| \rvw_\ell$ to have a spherical rotation-invariant distribution is when  
$$p\prnt{\left.\inp{\rvwt_\ell}{ \rvv_1}\right| \inp{\rvwt_\ell}{ \rvv_2}, \rvw_\ell} \stackrel{d}{=} p\prnt{\left.-\inp{\rvwt_\ell}{ \rvv_1}\right| \inp{\rvwt_\ell}{\rvv_2}, \rvw_\ell},$$ 
for any pair of perpendicular vectors $\rvv_1 \neq 0$ and $\rvv_2 \neq 0$. 

Consider the model in \cref{eq: quantization to rotation},  any orthogonal transformation $\rmU(\rtheta_\ell \big| \rvw_\ell)$ can be represented by an orthonormal basis, obtained by the  Gram-Schmidt process. That is, finding two orthonormal vectors $\rvu_1$ and $\rvu_2$ that span the plane of rotation generated by $\rvw_\ell$ and some $\rvw^\prime_\ell$ that is $\rtheta_\ell$ away from $\rvw_\ell$, and then, extend this basis to $\R^{n_\ell}$. This allows us to consider the rotation  in the plane generated by those vectors, with respect to the extended basis \cite{598782}. Accordingly,  let $\rvu_1 = \frac{\rvw_\ell}{\Vert \rvw_\ell \Vert}$ and $\rvu_2 = \frac{\rvw^\prime_\ell - \langle \rvu_1, \rvw^\prime_\ell \rangle \rvu_1 }{\Vert \rvw^\prime_\ell - \langle \rvu_1, \rvw^\prime_\ell \rangle \rvu_1  \Vert}$, then \RB{add drawing.}
\begin{equation}
    \rmU(\rtheta_\ell \big| \rvw_\ell) = \rmI_{n_\ell} - \rvu_1\rvu_1^{\etT} - \rvu_2 \rvu_2^{\etT} + \brkt{\rvu_1 , \rvu_2} \rmR_{\rtheta_\ell} \brkt{\rvu_1 , \rvu_2}^\etT,
    \label{eq: rotation u}
\end{equation}
where $\rmI_{n_\ell}$ is the $n_\ell\times n_\ell$ identity matrix and $\rmR_{\rtheta_\ell}$ is the rotation matrix
\[
 \rmR_{\rtheta_\ell} =
  \left[ {\begin{array}{cc}
    \cos(\rtheta_\ell) & -\sin(\rtheta_\ell) \\
    \sin(\rtheta_\ell) & \cos(\rtheta_\ell) \\
  \end{array} } \right],
\]
that rotates at a scalar angle $\rtheta_\ell$, and $\brkt{\rvu_1 , \rvu_2}$ is $n_\ell \times 2$ matrix whose columns are $\rvu_1$ and $\rvu_2$, respectively.  Plugging \cref{eq: rotation u} to \cref{eq: quantization to rotation}, and noting that $\frac{\rvw_\ell}{\Vert \rvw_\ell \Vert} = \rvu_1$, we obtain
 \begin{equation}
     \rvwt_\ell = \Vert \rvwh_\ell \Vert \cdot \prnt{\cos(\rtheta_\ell) \rvu_1 + \sin(\rtheta_\ell)\rvu_2} 
     \label{eq: rvwh ell}
 \end{equation}
To simplify notation, let  $\rvu \triangleq \prnt{\cos(\rtheta_\ell) \rvu_1 + \sin(\rtheta_\ell)\rvu_2}$, and note that for any perpendicular pair $\rvv_1, \rvv_2$, the vector $\rvu$ can be decomposed to $\rvu = \rvu^\parallel + \rvu^\perp$, where $\rvu^\parallel$ resides in the plane generated by $\rvv_1$ and $\rvv_2$, and $\rvu^\perp$ resides in the null-space of this plane. Hence, 
\begin{equation}
     \rvwt_\ell = \Vert \rvwh_\ell \Vert \cdot (\rvu^\parallel + \rvu^\perp) 
     \label{eq: rvwh ell simple}
 \end{equation}

Accordingly, we have
\begin{align}
    & p\prnt{\left.\inp{\rvwt_\ell}{ \rvv_1}\right| \inp{\rvwt_\ell}{ \rvv_2}, \rvw_\ell} &\\
    %&\stackrel{(a)}{=}p\prnt{\left.\inp{\Vert \rvwh_\ell \Vert \cdot \rvu}{ \rvv_1} \right| \inp{\Vert \rvwh_\ell \Vert \cdot \rvu}{\rvv_2 }, \rvw_\ell}&\nonumber\\
    & \stackrel{(a)}{=} p\prnt{\left.\inp{\Vert \rvwh_\ell \Vert \cdot (\rvu^\parallel + \rvu^\perp)}{ \rvv_1} \right| \inp{\Vert \rvwh_\ell \Vert \cdot (\rvu^\parallel + \rvu^\perp)}{\rvv_2 }}&\nonumber\\
    & \stackrel{(b)}{=} p\prnt{\left.\inp{\Vert \rvwh_\ell \Vert \cdot \rvu^\parallel}{ \rvv_1} \right| \inp{\Vert \rvwh_\ell \Vert \cdot \rvu^\parallel}{\rvv_2 }}&\nonumber\\
   &\stackrel{(c)}{=} p\prnt{\left.\Vert \rvwh_\ell \Vert \cdot \Vert \rvu^\parallel \Vert \cdot  \cos(\alpha) \right| \Vert \rvwh_\ell \Vert \cdot \Vert \rvu^\parallel \Vert  \cdot \sin(\alpha)}&\nonumber\\
   &\stackrel{(d)}{=} p\prnt{\left.\Vert \rvwh_\ell \Vert \cdot \Vert \rvu^\parallel \Vert \cdot \cos(\alpha) \right| \Vert \rvwh_\ell \Vert \cdot \Vert \rvu^\parallel \Vert \cdot \sin(\alpha)}&\nonumber\\
%   &\stackrel{(e)}{=} p\prnt{\left.\Vert \rvwh_\ell \Vert \cdot \cos(\pi - \tilde{\alpha}) \right| \Vert \rvwh_\ell \Vert \cdot \sin(\tilde{\alpha})}&\nonumber\\
%   &\stackrel{(f)}{=} p\prnt{\left.-\Vert \rvwh_\ell \Vert \cdot \cos( \tilde{\alpha}) \right| \Vert \rvwh_\ell \Vert \cdot \sin(\tilde{\alpha})}& \nonumber \\
%   & = p\prnt{-\left.\inp{\rvwh_\ell}{ \rvv_1}\right| \inp{\rvwh_\ell}{ \rvv_2}}
\end{align}
where (a) follows by \cref{eq: rvwh ell simple}. (b) follows by the linearity and since $\rvu^\perp$ is perpendicular to both $\rvv_1$ and $\rvv_2$ (c) follows due to the orthogonality of the basis $\rvv_1$ and $\rvv_2$, where $\alpha$ is the angle between $\rvu^\parallel$ and $\rvv_1$. (d) follows by a trigonometric identity for the sine function. (e) follows by changing variables, such that $\tilde{\rtheta}_\ell = \pi - \rtheta_\ell$. (f) follows by a trigonometric identity for the cosine function. 
 Thus, \Cref{prop: rotation invariance of rvwh}  follows. %holds for any  $\rtheta_\ell$. Moreover, the rotation-invariant spherical distribution emerges also when conditioning over $\rvw_\ell$. Hence, \Cref{prop: rotation invariance of rvwh} follows.
\end{proof}
